Efficient Knowledge Distillation via Curriculum Extraction

Knowledge distillation is a technique used to train a small student network using the output generated by a large teacher network, and has many empirical advantages~\citep{Hinton2015DistillingTK}. While the standard one-shot approach to distillation only uses the output of the final teacher network, recent work~\citep{panigrahi2024progressive} has shown that using intermediate checkpoints from the teacher's training process as an implicit ``curriculum'' for progressive distillation can significantly speed up training. However, such schemes require storing these checkpoints, and often require careful selection of the intermediate checkpoints to train on, which can be impractical for large-scale training. In this paper, we show that a curriculum can be \emph{extracted} from just the fully trained teacher network, and that this extracted curriculum can give similar efficiency benefits to those of progressive distillation. Our extraction scheme is natural; we use a random projection of the hidden representations of the teacher network to progressively train the student network, before training using the output of the full network. We show that our scheme significantly outperforms one-shot distillation and achieves a performance similar to that of progressive distillation for learning sparse parities with two-layer networks, and provide theoretical guarantees for this setting. Additionally, we show that our method outperforms one-shot distillation even when using transformer-based architectures, both for sparse-parity learning, and language modeling tasks.

==> JL-student-training.tex <==
\section{Student Training}


In this section, we analyze our student training algorithm (\Cref{alg:2_stage_training_student}). The student algorithm differs from the teacher training algorithm only in the first phase, where we use the distillation loss \(\ell_{DL}(\bx, f, g) := -f(\bx) \cdot g(\bx)\). Here, \(f = f_s^{(1)} \in \R^{m_s}\) is the first layer of the student network, and \(g = Af_t^{(1)}(\bx)  \in \R^{m_s}\) is the first layer of the teacher network projected to the student's hidden layer dimension.

\begin{theorem}
% Let $S\subseteq [d]$ be a fixed subset with $|S|=k$, and define the parity function on $\{\pm1\}^d$ by 
% $ \operatorname{parity}(x)=\prod_{j\in S} x_j.$
Assume that for each $x\in\{\pm1\}^d$ there is a hidden representation $v(x)\in\mathbb{R}^{m_t}$ and a fixed vector $u\in\mathbb{R}^{m_t}$ satisfying 
$ \langle v(x),u\rangle=\operatorname{parity}(x).$

Let $R\in\mathbb{R}^{m_s\times m_t}$ be a random projection matrix that satisfies the Johnson--Lindenstrauss (JL) property; that is, for any fixed $w\in\mathbb{R}^{m_t}$ and any $0<\epsilon<1$ we have 
$ \Pr\Bigl[\bigl|\|Rw\|^2-\|w\|^2\bigr|\ge\epsilon\,\|w\|^2\Bigr]\le2\exp\Bigl(-c\,\epsilon^2\,m_s\Bigr),$
for some universal constant $c>0$. 

Then, if 
$ m_s\ge\frac{C\,(d+\ln(1/\delta))}{\epsilon^2},$
for some constant $C>0$, it follows that with probability at least $1-\delta$ the following holds for all $x\in\{\pm1\}^d$:
$\Bigl|\langle Rv(x),Ru\rangle-\langle v(x),u\rangle\Bigr|\le\epsilon\,\|v(x)\|\|u\|.$
In particular, since $\langle v(x),u\rangle=\operatorname{parity}(x)$, we have for all $x\in\{\pm1\}^d$
$$
\langle Rv(x),Ru\rangle=\operatorname{parity}(x)\pm\epsilon\,\|v(x)\|\|u\|.
$$
\end{theorem}

\begin{proof}
There are at most $2^d$ distinct vectors $v(x)$ as $x$ ranges over $\{\pm1\}^d$. Let $X$ be this set, so that $|X|\le2^d$.

For any fixed $x\in X$ and any fixed $w\in\{v(x),\, u,\, v(x)+u,\, v(x)-u\}$ the JL property guarantees that 
$ (1-\epsilon)\|w\|^2\le\|Rw\|^2\le(1+\epsilon)\|w\|^2, $
with probability at least 
$ 1-2\exp(-c\,\epsilon^2\,m_s). $
Since the set 
$ W=\{v(x),\, u,\, v(x)+u,\, v(x)-u : x\in X\} $
has cardinality at most $4|X|\le4\cdot2^d$, by the union bound the above inequality holds for all $w\in W$ simultaneously with probability at least 
$ 1-8\cdot2^d\exp(-c\,\epsilon^2\,m_s). $
Thus, if 
$ m_s\ge\frac{C\,(d+\ln(1/\delta))}{\epsilon^2}, $
for a sufficiently large constant $C$, then with probability at least $1-\delta$ the JL property holds for every vector in $W$.

Using the polarization identity, for any fixed $x\in X$ we have 
$$
\langle v(x),u\rangle=\frac{1}{4}\Bigl(\|v(x)+u\|^2-\|v(x)-u\|^2\Bigr).
$$
Similarly,
$$
\langle Rv(x),Ru\rangle=\frac{1}{4}\Bigl(\|R(v(x)+u)\|^2-\|R(v(x)-u)\|^2\Bigr).
$$
Thus, for any fixed $x\in X$,
\begin{align*}
\Bigl|\langle Rv(x),Ru\rangle-\langle v(x),u\rangle\Bigr|
&\le\frac{1}{4}\Bigl(\bigl|\|R(v(x)+u)\|^2-\|v(x)+u\|^2\bigr|+\bigl|\|R(v(x)-u)\|^2-\|v(x)-u\|^2\bigr|\Bigr)\\[1mm]
&\le\frac{1}{4}\Bigl(\epsilon\,\|v(x)+u\|^2+\epsilon\,\|v(x)-u\|^2\Bigr)\\[1mm]
&=\frac{\epsilon}{4}\Bigl(\|v(x)+u\|^2+\|v(x)-u\|^2\Bigr).
\end{align*}
Note that 
$$
\|v(x)+u\|^2+\|v(x)-u\|^2=2\|v(x)\|^2+2\|u\|^2.
$$
Thus,
$$
\Bigl|\langle Rv(x),Ru\rangle-\langle v(x),u\rangle\Bigr|\le\frac{\epsilon}{2}\Bigl(\|v(x)\|^2+\|u\|^2\Bigr).
$$
A standard, slightly sharper analysis shows that we can obtain 
$$
\Bigl|\langle Rv(x),Ru\rangle-\langle v(x),u\rangle\Bigr|\le\epsilon\,\|v(x)\|\|u\|.
$$

Since this bound holds for every fixed $x\in X$ and $|X|\le2^d$, the union bound implies that with probability at least $1-\delta$ it holds simultaneously for all $x\in\{\pm1\}^d$. In particular, for all $x\in\{\pm1\}^d$ we have 
$$
\langle Rv(x),Ru\rangle=\operatorname{parity}(x)\pm\epsilon\,\|v(x)\|\|u\|.
$$
\end{proof}

This shows that for a relatively small sized student network, it is possible to project the teacher down while still having a good correlation. We now have to verify that the minimizer of the first stage is actually able to match the projected teacher outputs, and that this property continues to hold.  


==> main-body-icml.tex <==
\section{Introduction}
In the era of large-scale models, as the cost of training state-of-the-art models increases substantially with each passing year, leveraging compute effectively for training and inference has become increasingly important. Knowledge distillation~\citep{Hinton2015DistillingTK} is one popular technique that is commonly used to reduce the amount of compute necessary for inference, by training a small \emph{student} network to mimic the output of a large teacher network. Indeed, several state-of-the-art language models are distilled versions of larger models~\citep{deepseekai2025deepseekr1incentivizingreasoningcapability,abdin2024phi4technicalreport,geminiteam2024gemini15unlockingmultimodal,openai-o1mini}.

\begin{figure}[t]
    \centering
    %--------------------
    % First subfigure
    %--------------------
    \begin{minipage}[b]{\linewidth}
        \centering
        \hspace{-.8cm}
        %\input{figs/curriculum_extraction_diagram}
        \scalebox{0.5}{\input{figs/curriculum_extraction_diagram}}
            \caption{%
    Our curriculum extraction method trains the student model in a layer-wise fashion. Student layers are sequentially aligned to a random projection of the corresponding teacher layer’s hidden representation using the Mean Squared Error (MSE). After aligning layers, the student is trained on the teacher’s output logits via the KL Divergence loss.}
            \label{fig:curriculum_extraction_diagram}
    \end{minipage}
    % \caption{%
    % Our curriculum extraction method trains the student model in a layer-wise fashion. Student layers are sequentially aligned to a random projection of the corresponding teacher layer’s hidden representation using the Mean Squared Error (MSE). After aligning layers, the student is trained on the teacher’s output logits via the KL Divergence loss.
    % \new{SK: Careful integration here}
    % \textbf{In-support and out-of-support correlations.} 
    % \new{in progress... }
     % A two-layer MLP trained on 100-dimensional 6-sparse parity data exhibits distinct in-support (red) and out-of-support (blue) correlations of $(Af_t^{(1)})(\bx)$ with $x_j$ for the random projection $A \in \R^{1 \times m_t}$. When $j$ is in the support, the correlations show significantly larger standard deviations compared to when $j$ is outside the support. 
        % }
\end{figure}

\begin{figure*}[t]
    \centering
    %--------------------
    % First subfigure
    %--------------------
    \begin{minipage}[t]{0.31\linewidth}
        \centering
            \hspace*{-2mm} % Adjust this negative space to control horizontal tightness
        \includegraphics[width=1.12\textwidth]{unpolished_figs/mlp_student_accuracy.pdf}
        %\vspace{0.5em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(a)} % Manually add caption
        \label{fig:mlp_student_accuracy}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.31\linewidth}
    \centering
        \hspace*{-3mm} % Adjust this negative space to control horizontal tightness
    \includegraphics[width=1.12\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
        %\vspace{0.5em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(b)} % Manually add caption
    \label{fig:transformer_student_accuracy}
    \end{minipage}
    \hfill
        \begin{minipage}[t]{0.31\linewidth}
    \centering
    \hspace*{-3mm} % Adjust this negative space to control horizontal tightness
    \includegraphics[width=1.12\textwidth]{unpolished_figs/student_wikipedia_accuracy.pdf}
        %\vspace{0.5em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(c)} % Manually add caption
    \label{fig:wiki}
    \end{minipage}
    \caption{%
    \textbf{Comparing Curriculum Extraction and One-Shot Distillation.}
     We show three tasks for which curriculum extraction outperforms one-shot distillation:
(a) A two-layer MLP trained on 100-dimensional 6-sparse parity, with a teacher hidden dimension of 50k and a student hidden dimension of 100.
(b) A transformer trained on 100-dimensional 6-sparse parity, using 256-dimensional embeddings, where the teacher has 32 attention heads and the student has 4.
(c) A BERT-large model fine-tuned on the Wikipedia dataset, with the teacher using 768-dimensional embeddings, 12 attention heads, and 12 transformer blocks, while the student reduces embeddings to 256 dimensions and attention heads to 4. The dashed vertical lines indicate the iterations where the layer being distilled is changed in the case of curriculum extraction, and a change in teacher checkpoint in the case of progressive distillation.}
    \label{fig:student_accuracies}
\end{figure*}

Despite the adoption of distillation for language model training, prior work~\citep{panigrahi2024progressive, anil2020largescaledistributedneural,mirzadeh2019improvedknowledgedistillationteacher} has shown that just using the output of the fully-trained teacher network to train the student can result in poor performance relative to the teacher (a ``teacher-student gap'' in performance), and that \emph{progressive distillation} can significantly improve the performance of the student. \citet{panigrahi2024progressive} in particular offers an explanation for this phenomenon -- the intermediate checkpoints during the training of the teacher network act as an implicit \emph{curriculum} for the training of the student network, with earlier checkpoints emphasizing simpler patterns (e.g., local syntax in the case of language models), and later checkpoints capturing complex abstractions (e.g., long-range semantics). Please see \Cref{sec:related_work} for a more detailed overview of related work. 

While progressive distillation offers significant efficiency advantages over one-shot distillation, it requires storing frequent checkpoints during the training of the teacher, which can be prohibitive for modern LLMs. Deciding on which checkpoints to make use of to train the student is often unclear; such checkpoints are found by extensive experimentation in the works listed above, which can be impractical. Moreover, in many cases, one lacks access to intermediate checkpoints during training, even for open-source models~\citep{jiang2023mistral7b,deepseekai2025deepseekr1incentivizingreasoningcapability,meta2024llama}, making progressive distillation impossible.

This raises a natural question -- can we design a scheme that maintains the advantages of progressive distillation without suffering from its drawbacks? Specifically, can we leverage the final fully-trained teacher model more effectively to train the student model efficiently?

\paragraph{Curriculum Extraction.} We propose a scheme to \emph{extract} a curriculum from the fully-trained teacher network. Our key insight is that the layer-wise hierarchy of a fully trained network naturally encodes a progression from simple to complex features. To operationalize this, we train the student's hidden layers sequentially on \emph{random projections} of the teacher’s hidden layers, starting from shallow (layer $l$, say) to deep (the final layer $L$), before training the full student network on the output of the full teacher network. See Figure~\ref{fig:curriculum_extraction_diagram} for a visual description of our extraction scheme.

 By progressively training on projections from shallower to deeper layers, the student learns incrementally—mirroring the coarse-to-fine learning in progressive distillation, without having to store intermediate checkpoints. Beyond circumventing checkpoint storage, our approach can potentially be applied to efficiently distill from open-source models (e.g., Llama~\citep{meta2024llama}, Mistral~\citep{jiang2023mistral7b}, and Deepseek models~\citep{deepseekai2025deepseekr1incentivizingreasoningcapability}), where only the final model is available. In addition, our method is computationally cheaper than one-shot or progressive distillation per training iteration  --  during early stages, only a subset of student and teacher layers are active, reducing memory and FLOPs per iteration.  

%XXX FLOPs??
%Formally, let the student network $f_\theta$ consist of the $L$ layers $\{s_1, \dots, s_L\}$, and similarly, let the tea when training using layer $k$, the student minimizes the MSE between $(1)$ the output of its layer $s_k$
\subsection{Our Results}

\paragraph{Sparse Parity Learning.}
We show that our curriculum extraction scheme is \emph{significantly} more efficient than one-shot distillation for the task of learning sparse parities using a two-layer MLP, and provide a theoretical analysis for this setting. See Section~\ref{sec:sparse_parities} for a formal description of sparse parity learning and two-layer MLPs. Here, we state an informal version of our main theorem, with the formal theorem stated in \Cref{sec:main-thm}.

\begin{theorem}[Main, Informal]
\label{thm:main_informal}
Let $d \geq \tilde \Omega(k^4)$. 
Consider learning $d$-dimensional $k$-sparse parity with a student model of size $\tilde{\Theta}(2^{O(k)})$, where $\tilde{O}, \tilde{\Theta}$ hides polylog factors in $d,k$. Suppose the teacher 
% (of size $2^{O(k)} \poly(d,k)$) 
has a loss $O(\epsilon)$ for some small $\epsilon > 0$. Then, the total sample complexity needed for the student to reach $\epsilon$-loss using curriculum extraction based on random projection is: $\tilde{\Theta}\left(2^{O(k)} \poly(d,k) \epsilon^{-2}\right)$. However, one-shot distillation requires at least $\Omega\left(d^{k-1} \epsilon^{-2}\right)$ samples.\end{theorem}

 Thus, one-shot distillation \emph{requires} $\Omega(d^{O(k)})$ samples to learn sparse parties, while our curriculum extraction scheme can learn using only $O(2^{O(k)} \poly(d))$ samples. 
We show in Figure~\ref{fig:student_accuracies} (a) that our curriculum extraction scheme significantly outperforms one-shot distillation empirically, as predicted by our theory -- our scheme succeeds in learning, while one-shot distillation fails after training using $2 \cdot 10^6$ samples. Furthermore, it has similar performance as progressive distillation for a carefully chosen checkpoint -- we choose the checkpoint during training of the teacher network whose output is most correlated with the support of the parity function, as proposed by~\citet{panigrahi2024efficient}.

We also show empirically that our scheme continues to outperform one-shot distillation when using a transformer-based architecture for learning sparse parities in Figure~\ref{fig:student_accuracies} (b).

\paragraph{Masked Language Modeling (BERT).}

In addition to learning sparse parities, we empirically study our curriculum extraction scheme for language modeling, focusing on BERT-style \emph{masked language modeling}. We study two settings with different kinds of data: (i) Synthetic data generated by a Probabilistic Context-free Grammar (PCFG), and (ii) Real-world language data from Wikipedia.

In the case of PCFGs, we show that our scheme outperforms one-shot distillation, both in terms of computational efficiency (number of FLOPs), and in terms of sample efficiency (number of iterations), in Figures~\ref{fig:pcfg_bert} (a) and (b). We also show that our curriculum scheme outperforms just using the final hidden representation of the teacher to distill before distilling using the full network; this suggests that the efficiency benefits of our scheme do indeed come from the fact that the layers of the teacher network implicitly act as a curriculum, rather than merely from the increased dimensionality of the distilled features.

For Wikipedia data, we show in Figure~\ref{fig:student_accuracies} (c) that curriculum extraction has a significant accuracy advantage over one-shot distillation when training for $24 \cdot 10^3$ iterations with a batch size of $128$ -- for extraction, we use $4$ intermediate layers to distill, before distilling with the full teacher network.

% \new{SK: put 3 figures -- wiki, sparse parity MLP, sparse parity transformer side by side. But we don't need to include synthetic BERT here, but should talk about how improvement is about flops. }

% \section{Related Work}
% \label{sec:related_work}

% % \paragraph{Knowledge Distillation and Progressive Training}  
% % Knowledge distillation (KD), pioneered by \citep{Hinton2015DistillingTK}, transfers knowledge from a computationally intensive teacher model to a lightweight student by aligning their output distributions. This paradigm has been widely adopted in language models to reduce inference costs, with techniques like sequence-level distillation \citep{kim2016sequence} further optimizing efficiency. For example, DistilBERT \citep{sanh2019distilbert} and TinyBERT \citep{jiao2020tinybert} demonstrate that students can retain $95–97\%$ of teacher performance while being significantly smaller.

% % Recent studies, however, reveal limitations in one-shot distillation, where students trained solely on the final teacher outputs underperform compared to progressive approaches. \citep{panigrahi2024progressive}  proposing progressive distillation via intermediate teacher checkpoints and attempts to provide an explanation for why the sample complexity of training the student model can potentially be much smaller by studying it theoretically in the context of learning sparse parities. 
% % % Similar findings appear in 
% % % vision \citep{yuan2021progressive} and 
% % % multilingual models \citep{wei2021consistent}, where phased training improves robustness. 
% % Reinforcement learning frameworks like \citep{schmitt2022kickstarting} further validate that mimicking a teacher’s learning trajectory accelerates student convergence.


% % \paragraph{Curriculum Learning and Extraction}  
% % Curriculum learning, formalized by \citep{bengio2009curriculum}, posits that structuring training data by difficulty improves model efficiency and generalization. Early applications in NLP used handcrafted curricula for tasks like machine translation \citep{kocmi2017curriculum}, while automated methods leverage self-paced learning \citep{kumar2010self} or reinforcement learning \citep{graves2017automated}. 
% % % For instance, \citep{guo2023curriculum} dynamically adjusts task complexity using meta-gradients, achieving state-of-the-art results on reasoning benchmarks.

% % A parallel line of work extracts implicit curricula from model internals. Studies like \citep{tenney2019bert} and \citep{hewitt2019structural} show that BERT’s layers encode hierarchical linguistic features, suggesting that intermediate representations could scaffold learning. However, these methods still require access to intermediate states, which are often unavailable.

% % Our work bridges this gap by proposing hidden-representation curriculum extraction, which synthesizes a curriculum from a fully trained teacher’s internal dynamics. This aligns with insights from \citep{shwartz2017opening,voita2019analyzing,aguilar2020knowledge,liang2023less}, who argue that intermediate layers encode structured knowledge hierarchies. 
% % % Our use of random projections to approximate these hierarchies draws inspiration from work on model compression \citep{ma2020unicoder} and low-rank adaptation \citep{hu2021lora}, but uniquely targets curriculum synthesis.

% % % Theoretical support for our technique comes from \citep{wei2022learning}, who prove that curriculum training accelerates parity learning—a task analogous to sparse parities. Similarly, \citep{abbe2023merged} analyze how phased training breaks symmetry in neural networks, providing a foundation for our theoretical guarantees.

% % \paragraph{Layer-Wise Distillation}




% % ---

% % \paragraph{Knowledge Distillation}  
% % Knowledge distillation (KD), pioneered by \citep{Hinton2015}, transfers knowledge from a computationally intensive teacher model to a lightweight student by aligning their output distributions. This paradigm has been widely adopted in language models to reduce inference costs, with techniques like sequence-level distillation \citep{kim2016sequence} further optimizing efficiency. For example, DistilBERT \citep{sanh2019distilbert} and TinyBERT \citep{jiao2020tinybert} demonstrate that students can retain $95$--$97\%$ of teacher performance while being significantly smaller.

% % Recent studies reveal limitations in one-shot distillation, where students trained solely on final teacher outputs underperform compared to progressive approaches. \citep{panigrahi2024progressive} proposes progressive distillation via intermediate teacher checkpoints and explains its efficiency theoretically in the context of learning sparse parities. Menon et al. \citep{Menon2021} formalize why teacher outputs (e.g., Bayes class probabilities) tighten generalization gaps, while \citep{Ren2022} addresses poor teacher calibration via moving-average supervision. The teacher’s guidance also provides regularization benefits, such as bias-variance control \citep{Zhou2020}, sparsity induction \citep{Mobahi2020}, or label smoothing \citep{Yuan2020}. Prior work on multi-step distillation \citep{Mobahi2020,Pareek2024} explores self-distillation (students becoming teachers), but focuses on regression tasks rather than classification.

% % Despite its promise, progressive distillation faces challenges:  
% % (1) Storing intermediate checkpoints for large models (e.g., Llama-3 \citep{meta2024llama}) incurs prohibitive costs;  
% % (2) Optimal intervals require heuristic tuning \citep{zhou2023lima};  
% % (3) Many models (e.g., GPT-4 \citep{openai2023gpt4}) only release final weights.  

% % \paragraph{Curriculum Learning}  
% % Curriculum learning, formalized by \citep{bengio2009curriculum}, structures training data by difficulty to improve efficiency. While early NLP work used handcrafted curricula \citep{kocmi2017curriculum}, modern methods automate this via self-paced learning \citep{kumar2010self} or model internals. Studies show BERT’s layers encode linguistic hierarchies \citep{tenney2019bert,hewitt2019structural}, suggesting intermediate representations scaffold learning—though these require checkpoint access \citep{shwartz2017opening,voita2019analyzing}.

% % \new{Theoretical support comes from $\Omega(dk)$ statistical query lower bounds for sparse parity learning (\citep{Edelman2023}), The fact that feature learning reduces sample complexity from $\Theta(d^2)$ to $O(d\ \text{polylog}\ d)$ for $k=2$ (\citep{Glasgow2024}) and the fact that neural networks outperform kernel methods on single-/multi-index functions (\citep{Abbe2022,Abbe2023}). 

% % These align with \citep{wei2022learning} on curriculum-driven parity acceleration and \citep{damian2024a} on neural feature representation. }

% % \paragraph{Layer-Wise Distillation}  
% % \new{XXX flip into Distillation, -- length to be noise distillation and curriculum learning.}

% % Layer-wise distillation extends knowledge transfer beyond the final output by aligning intermediate representations between teacher and student networks. The foundational work of \citep{romero2015fitnets} introduced "hint layers," forcing student layers to mimic teacher activations through regressors. This approach demonstrated that intermediate supervision accelerates convergence, particularly when student depth differs from teachers \citep{kim2021dynamic}.

% % Modern implementations leverage diverse alignment strategies:  
% % (1) \textbf{Feature matching}: Minimizing L2 distances between layer outputs \citep{yim2017gift} or Gram matrices \citep{li2017learning};  
% % (2) \textbf{Attention transfer}: Aligning spatial attention maps in vision models \citep{zagoruyko2016paying} or self-attention distributions in transformers \citep{tian2020contrastive};  
% % (3) \textbf{Prediction consistency}: Enforcing layer-wise label predictions \citep{guo2020online} via multiple classifiers.  

% % Recent theoretical analyses by \citep{shi2022layer} reveal that layer alignment provides implicit curriculum benefits - shallower student layers learn low-level features (e.g., edge detectors) before deeper layers combine them into high-level concepts. This aligns with biological learning patterns observed in \citep{lampinen2021training}, where hierarchical feature acquisition mirrors human skill development. For transformer architectures, \citep{jiao2020tinybert} shows that layer-wise distillation improves positional encoding transfer, while \citep{turc2019wellread} shows layer pruning via importance scoring.

% % Key challenges persist:  
% % - \textbf{Architectural mismatch}: Requires adaptive projection when layer dimensions differ \citep{ahn2019uncertainty};  
% % - \textbf{Optimization conflict}: Layer losses may compete with final task objective \citep{passalis2018heterogeneous};  
% % - \textbf{Computational overhead}: $25-40\%$ increased memory from multi-layer comparisons \citep{xu2020knowledge}.  

% % Our work connects to layer-wise paradigms through hidden-representation curriculum extraction, but eliminates layer alignment costs by using random projections rather than direct matching. 
% % We synthesize a curriculum from the internal dynamics of a fully trained teacher. This aligns with insights from \citep{shwartz2017opening,voita2019analyzing,aguilar2020knowledge,liang2023less}, who argue that intermediate layers encode structured knowledge hierarchies. Unlike \citep{zhou2020bertic}, which requires full layer access, our method synthesizes progressive curricula from final model states.

% \paragraph{Knowledge Distillation}  
% Knowledge distillation (KD), pioneered by \citep{Hinton2015DistillingTK}, transfers knowledge from computationally expensive teacher models to lightweight students by aligning output distributions. This paradigm has been widely adopted in modern language models for inference cost reduction. Examples of models trained via distillation include ChatGPT O1-mini~\citep{openai-o1mini}, Gemini Flash~\citep{geminiteam2024gemini15unlockingmultimodal}, and the Phi series of models~\citep{abdin2024phi4technicalreport}. Despite the success of distillation, there have been a number of works~\citep{mirzadeh2019improvedknowledgedistillationteacher,cho,supervision_complexity,panigrahi2024progressive} that have observed that simply distilling using the output of the fully trained teacher network can be suboptimal, resulting in a ``teacher-student gap'' in capabilities. To circumvent this gap, these works have proposed \emph{progressive distillation}, a technique that trains the student using intermediate checkpoints during the teacher training progressively, before training on the output of the fully-trained teacher. \citep{panigrahi2024progressive} proposes that the intermediate checkpoints act as an implicit \emph{curriculum}, allowing the student to learn simpler functions before moving to the final complex one, and shows theoretical and empirical evidence to support these claims.%In this work, we propose a method for extracting a similar curriculum from the fully-trained teacher network, and similar to \citep{panigrahi2024progressive}, we show rigorous guarantees for sparse parity learning with two-layer MLPs, and empirical results in sparse parity and language model settings. 


%  Despite its promise, progressive distillation faces some challenges -- (1) storing intermediate checkpoints for large models incurs prohibitive costs, (2) finding an effective checkpoint schedule to use is done heuristically \citep{panigrahi2024progressive}, requiring costly trial-and-error, (3) Most models, including open-source ones (e.g., Llama 3~\citep{meta2024llama}, Mistral~\citep{jiang2023mistral7b}) only release final weights, making progressive distillation impossible.

%  %To mitigate these issues, recent work explores memory-efficient distillation via parameter recycling \citep{xia2022meta} or gradient matching \citep{zhu2023dynamic}, but these methods still rely on checkpoint access.
 
% Our method builds a curriculum using just the fully-trained teacher network, and thus, avoids the shortcomings or progressive distillation. While our curriculum extraction method is related to layer-wise distillation methods proposed in the literature~\citep{aguilar2020knowledge, liang2023less, jiao2020tinybert,Sun2019PatientKD}, these methods typically require the teacher and student to have the same embedding dimension. In contrast, our method uses a \emph{random projection} to embed the teacher's hidden representation into the student's embedding dimension, allowing us to accommodate differing embedding dimensions. Our method also crucially relies on the stage-wise curriculum extraction of each layer individually, while the aforementioned works typically distill teacher layers simultaneously with the final output. Moreover, all of these works are heuristic in nature; we provide rigorous guarantees showing the correctness of our method, albeit in a stylized setting. 

% %This paradigm has been widely adopted in language models for inference cost reduction. 
% %For example, DistilBERT \citep{sanh2019distilbert} and TinyBERT \citep{jiao2020tinybert} demonstrate that students retain $95$--$97\%$ of teacher performance at significantly smaller scales. 
% %Layer-wise extensions of KD align intermediate representations through strategies like ``hint layers" \citep{romero2015fitnets}, feature matching via L2 distances \citep{yim2017gift}, attention transfer \citep{zagoruyko2016paying}.
% %% , or prediction consistency \citep{}. 
% %
% %Recent studies highlight limitations in one-shot distillation, where students trained solely on final teacher outputs underperform compared to progressive approaches. 
% %\citep{panigrahi2024progressive} proposes progressive distillation via intermediate checkpoints, theoretically explaining its efficiency for sparse parity learning. Menon et al. \citep{Menon2021} formalize how teacher outputs (e.g., Bayes class probabilities) tighten generalization gaps, while \citep{Ren2022} addresses poor teacher calibration via moving-average supervision. Teacher guidance also provides regularization benefits: bias-variance control \citep{Zhou2020}, sparsity induction \citep{Mobahi2020}, and label smoothing \citep{Yuan2020}. Prior work on multi-step distillation \citep{Mobahi2020,Pareek2024} explores self-distillation (students becoming teachers) but focuses on regression tasks. 
% %% Key challenges include (1) architectural mismatch requiring adaptive projections \citep{ahn2019uncertainty}, (2) optimization conflicts between layer losses and task objectives \citep{passalis2018heterogeneous}, and (3) $25$--$40\%$ computational overhead from multi-layer comparisons \citep{xu2020knowledge}.  
% %
% %Progressive distillation faces additional hurdles: storing intermediate checkpoints for large models (e.g., Llama-3 \citep{meta2024llama}) incurs prohibitive costs, optimal intervals require heuristic tuning \citep{zhou2023lima}, and many models (e.g., GPT-4 \citep{openai2023gpt4}) only release final weights. Our work connects to layer-wise paradigms through hidden-representation curriculum extraction but eliminates alignment costs via random projections. This synthesizes curricula from fully trained teachers, aligning with insights from \citep{shwartz2017opening,voita2019analyzing} on structured knowledge hierarchies in intermediate layers.
% %% , unlike \citep{zhou2020bertic} requiring full layer access.  
% %
% \paragraph{Curriculum Learning}  
% Curriculum learning, formalized by \citep{bengio2009curriculum}, structures training data by difficulty to improve learning efficiency. Early NLP work relied on handcrafted curricula \citep{kocmi2017curriculum}, while modern approaches automate this process through self-paced learning \citep{kumar2010self}. Recent advances, such as those by \citep{panigrahi2024efficient}, demonstrate that stagewise pretraining via incremental subnetworks achieves computational efficiency without compromising model quality, further supporting the benefits of progressive learning paradigms. Additionally, studies on BERT reveal that its layers encode linguistic hierarchies \citep{tenney2019bert,hewitt2019structural}, suggesting that intermediate representations can scaffold learning—though this typically requires access to intermediate checkpoints \citep{shwartz2017opening,voita2019analyzing}.
% %

% %Theoretical foundations for curriculum learning include $\Omega(dk)$ statistical query lower bounds for sparse parity learning \citep{Edelman2023}, the reduction of sample complexity from $\Theta(d^2)$ to $O(d\ \text{polylog}\ d)$ for $k=2$ through feature learning \citep{Glasgow2024}, and the superiority of neural networks over kernel methods in learning single- and multi-index functions \citep{Abbe2022,Abbe2023}. These findings align with insights into neural feature representation \citep{damian2024a} and the biological parallels of curriculum learning, where hierarchical feature acquisition mirrors human skill development \citep{lampinen2021training}.
% % while \citep{turc2019wellread} demonstrates layer pruning via importance scoring.  

\input{related-work}

\section{Curriculum Extraction}

We now describe our curriculum extraction scheme formally.

\begin{definition}[Curriculum Extraction Scheme]
\label{def:scheme}
Given a pre-trained teacher network $~T$ and a student network $S$, both having the same number of layers $L$, let $T_i$ and $S_i$ denote the network up to layer $i$ ($T_i:\R^{d} \rightarrow \R^{m_i}$ and $S_i:\R^{d} \rightarrow \R^{n_i}$).
Suppose also that for some $\ell \in [0, L)$ we are given a sequence $\{t_\ell, \dots, t_L\}$ such that $t_i \in \Z$ indicates the number of iterations we train $S_i$ for.
The Layer-Wise Curriculum Extraction Scheme proceeds as follows:

\begin{enumerate}
    \item \textbf{Initialization:} 
    Initialize the student network $S$ with random weights.
    \item \textbf{Layer-Wise Training:}
     For each $i \in [\ell, L-1]$, such that $t_i > 0$:
        \begin{enumerate}
            \item Define a random projection matrix $P_i : \R^{m_i} \rightarrow \R^{n_i}$ for layer $i$.
            \item Train \(S_i\) for \(t_i\) iterations to reduce the MSE loss between \(S_i(x)\) and \(P_i(T_i(x))\):
            $\mathcal{L}_i = \frac{1}{T} \sum_{t=1}^{T} \| S_i(x^{(t)}) - P_i(T_i(x^{(t)})) \|^2_2$
            where $T$ is the number of training samples.
        \end{enumerate}
    \item 
    Train the entire student network $S$ for $t_L$ iterations to reduce the KL-divergence loss between $S(x)$ and $T(x)$.
\end{enumerate}
\end{definition}



\section{Learning Sparse Parities via Curriculum Extraction}
\label{sec:sparse_parities}


To demonstrate the effectiveness of our curriculum extraction scheme, we study its performance in learning sparse parities. 
We compare our curriculum extraction scheme to one-shot distillation, where the student is trained directly on samples generated by the teacher. 
%In \Cref{subsec:prelims} we define the problem and our setup.
%In \Cref{subsec:proof_overview} we give a brief overview of the proof. 
%In \Cref{subsec:sparse_parity_experiments} we demonstrate our experimental results on transformer and MLP architectures. 
% we will briefly present our main theorem (a formal version of \Cref{thm:main_informal}) and outline the proof. 

% We also study this experimentally by training MLP and transformer models.

%\subsection{Theoretical Analysis}

\subsection{Preliminaries}
\label{subsec:prelims}

% We study the performance of our curriculum extraction scheme in the stylized context of learning the problem of sparse parities as defined in \Cref{prob:sparse_parities}. 
For our arguments in this section, we will assume WLOG that the support of the unknown parity is $S = [k]$. 
We will learn two-layer MLP networks of the form 
$f(\bx) := \ba \cdot \sigma(\bW \bx + \bb) = \sum_{i=1}^m a_i \sigma(\bw_i \cdot \bx + b_i)$. 
where $\bx \in \R^d; \bW \in \R^{d \times m}$; $\bb, \ba \in \R^m$, and $\sigma(t) := \max(0, t)$ is applied coordinate-wise when applied to a vector. 
We will denote the student network by $f_s$ and the teacher network by $f_t$ with hidden dimensions $m_s$ and $m_t$ respectively.
In general $m_s \leq m_t$. 
Let $\ell_f(\bx, y) := \max(0, 1-f(\bx)y)$ be the hinge loss. 
Our main task will be to find the best fitting two-layer MLP to an unknown sparse parity function. 

\begin{problem}[Learning Sparse Parities]
\label{prob:sparse_parities}
    Let \( S \subset [d] \) with \( |S| = k \) and \( k < d \) denote the support of our unknown sparse parity. 
    For \( \bx \in \{\pm 1\}^d \), we define $\chi_S(\bx) := \prod_{i \in S} x_i$ to be a \emph{sparse parity} supported on $S$.  
    Given a tolerance \(\epsilon \in \R\) and $n$ samples \(\{(\bx_i, \chi_S(\bx_i)) \mid \bx_i \sim_{u.a.r} \{\pm 1\}^d \text{ for } i \in [0, n]\}\) for an unknown support $S$, 
    the task of learning a sparse parity function using a two-layer MLP, is to find a two-layer MLP that achieves loss $\E_{(\bx, y)} [\ell_f(\bx,y)] \leq \epsilon$. 
\end{problem}


For our theoretical analysis, our training setup differs slightly from \Cref{def:scheme} when it comes to our losses -- we use a regularized version of the hinge loss to train the bottom layer of the teacher, the hinge loss to train the top layer of the teacher as well as the student, and a regularized version of a correlation-based distillation loss (defined below) to train the student's hidden layer.

\paragraph{Initialization}
Prior to training, we will initialize the network using the following symmetric initialization from \citet{barak2022hidden}.

\begin{definition}[Symmetric Initialization]
\label{def:sym_initialization}
Let $f(\bx) := \sum_{i=1}^m a_i \sigma(\bw_i \cdot \bx + b_i)$ be a two-layer MLP with input dimension $d$ and hidden dimension $m$. For each 
$1 \leq i \leq m/2,$ we initialize the parameters $\{\bw_i\}_{i=1}^m$, $\{b_i\}_{i=1}^m$ and $\{a_i\}_{i=1}^m$ as follows: $\bw_i \sim U(\{\pm 1\}^d),$
$b_i \sim U\left(\left\{-1 + \frac{1}{k}, \cdots, 1 - \frac{1}{k}\right\}\right), 
\quad a_i \sim U\left(\left\{\frac{\pm 1}{m}\right\}\right)$, $m/2 < i \leq m$ are set to $\bw_i = -\bw_{i -m/2}, \quad b_i = b_{i -m/2}, \quad a_i = -a_{i -m/2}$.
\end{definition}


\paragraph{Training Algorithms:}
We train the teacher network $f_t$ by minimizing the hinge loss in two stages. 
In the first stage of training, we freeze the top layer weights $(\ba)$ and train the network with a regularized version of $\ell_{f_t}(\bx, y)$, given by $\ell_{f_t}(\bx, y) - \lambda \|\bW\|^2$ updating only $\bW$.
In the second stage of training, we freeze the bottom layer weights and biases $\bW, \bb$ and only update $\ba$. 

For the student network $f_s$, we define a \emph{distillation loss} instead.
Let $f_t^{(1)} := \sigma(\bW \bx + \bb) : \R^d \rightarrow \R^{m_t}$ denote the output of the first layer of the teacher and suppose $A \in \R^{m_t \times m_s}$ is a random symmetric projection which mimics the initialization, i.e. for $i \leq m_t/2$, each \new{$A_{ij} \sim U(\{\pm 1/m_t\})$} and for $i > m_t/2$, 
$A_{ij} = -A_{(i-m/2)~j}$.
In the first stage (where we only update the bottom layer weights), the first layer of the student (i.e. $f_s^{(1)}(\bx) := \sigma(\bW_s \bx + \bb_s)$) is trained using the a similarly regularized version of the following distillation loss: 
$\ell_{DL}(\bx, f_s^{(1)}, Af_t^{(1)}) = \new{-f^{(1)}_s(\bx) \cdot (Af^{(1)}_t(\bx))}$, i.e. we use the loss $\ell_{DL}(\bx, f_s^{(1)}, Af_t^{(1)}) - \lambda \|\bW_s\|^2$ for a carefully chosen value of $\lambda$.
% \max(0, 1 - f^{(1)}_s(\bx) \cdot (Af^{(1)}_t(\bx))).

The second layer of the student ($\ba_s$) is then trained using the standard hinge loss.

\subsection{Theoretical Results}
\label{sec:main-thm}
We prove that, compared to one-shot distillation—where the student needs at least \(\Omega\left(d^{k-1}\right)\) samples to learn the unknown sparse parity—our curriculum extraction method reduces this requirement to \(\tilde{O}(2^{O(k)}\poly(k,d))\).
We state this formally below:
\begin{theorem}[Curriculum Extraction Requires Fewer Samples]
\label{thm:main}
    Let $m_s$ and $m_t$ denote the student and teacher hidden dimensions, with $m_t \geq m_s$ and $d \geq\tilde \Omega(k^4)$.
    Suppose the teacher model 
    % (having a hidden dimension of size $m_t$)
    % \new{(of size $O(2^{O(k)}\poly(d, k))$)} 
    has been trained to learn a $d$-dimensional $k$-sparse parity with the 2-stage training algorithm in \Cref{alg:2_stage_training},
    % , which satisfies the conditions in \Cref{lem:effect_of_1_step_on_w} at the end of the first stage 
    % \new{for hidden layer size $m_t \leq d^{k-1}$} 
    and achieves a loss of $\eps = O(d^{-c})$ for some constant $c \geq 1$ at the end of the second stage. 
    Suppose further, that we train a student model $f_s$ of size $m_s = \tilde{\Theta}(2^k k)$ using the following two strategies:
\begin{enumerate}
    \item \textbf{Random-projection curriculum extraction:} 
    Train the first layer of the student with a random projection of the first layer of the teacher to the right output dimension, and then train the entire student network with the final teacher network.
    \item \textbf{One-shot Distillation:} Train with the teacher network throughout.
\end{enumerate}

Then,
\begin{enumerate}
    \item 
    \label{item:sufficient_our_distillation_scheme}
    Under our distillation scheme, the total sample complexity to reach a loss of $\epsilon$ with probability $99\%$ is 
    % $\Theta(2^{O(k)} \poly(d,k)\epsilon^{-2} \log(k/\delta\epsilon)).$
    $\Theta(2^{O(k)} \poly(d,k)\epsilon^{-2} \log(k/\epsilon)).$
    \item The necessary sample complexity under distillation is at least
    \label{item:necessary_one_shot_distill}
    $\Omega\left(d^{\min(2c, k-1)}\right)$.
    
\end{enumerate}
% Then, (1) Under our distillation scheme, the total sample complexity to reach a loss of $\epsilon$ with probability $1 - \delta$ is $\Theta(2^{O(k)} d^2 \epsilon^{-2} \log(k/\delta\epsilon)).$ (2) The necessary sample complexity under distillation is at least
    % $\Omega\left(d^{\min(2c, k-1)}\right)$.
\end{theorem}
 The key difference between the two is that, in one-shot distillation, the student must identify one of \(\Omega(d^k)\) possible parity functions from scratch. In contrast, our scheme splits the learning into two phases: identifying the support and learning the final function. Initially, the gradients of the distillation loss guide the student in detecting the support of the sparse parity via the bottom layer. With the support identified, the student only needs to select from \(O(2^k)\) possible parities.

\subsubsection{Proof Overview}
\label{subsec:proof_overview}

\begin{figure}[t]
     \begin{minipage}[b]{\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{unpolished_figs/mlp_correlation.pdf}
        \caption{\textbf{In-support and out-of-support correlations.} 
    % \new{in progress... }
     A two-layer MLP trained on 100-dimensional 6-sparse parity data exhibits distinct in-support (red) and out-of-support (blue) correlations of $(Af_t^{(1)})(\bx)$ with $x_j$ for the random projection $A \in \R^{1 \times m_t}$. When $j$ is in the support, the correlations show significantly larger standard deviations compared to when $j$ is outside the support. }
        \label{fig:correlation_plot}
    \end{minipage}
\end{figure}

% In this section, we prove our main theorem which states that, compared to one-shot distillation—where the student requires at least $\Omega\left(d^{\min(2c, k-1)}\right)$ samples to learn the unknown sparse parity—our curriculum extraction method reduces the sample requirement to $\tilde O(2^{2k})$.

% To understand why this is the case, consider the difference in what the student must learn between the two situations. With one-shot distillation, the student has to learn one of $\Omega(d^k)$ possible parity functions that the teacher could be approximating and must identify the correct one from scratch.
% , greatly reducing the required sample size.
% \new{SK: Integrate this difference again into the rest, labels are broken now.}
% \new{SK: Fix algorithm enviornment in appendix.}
% \new{SK: Fix prose to connect with fact we don't have to main theorem.}

% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     \begin{minipage}[b]{0.5\linewidth}
%         \centering
%         \includegraphics[width=1\textwidth]{unpolished_figs/mlp_correlation.pdf}
%         % \caption{(a)}
%         \label{fig:mlp_correlation}
%     \end{minipage}
%     % \begin{minipage}[b]{0.8\linewidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
%     % \caption{MLP Student Accuracy}
%     % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     % \hfill
%     \caption{%
%     \textbf{In-support and out-of-support correlations.} 
%     % \new{in progress... }
%      A two-layer MLP trained on 100-dimensional 6-sparse parity data exhibits distinct in-support (red) and out-of-support (blue) correlations of $(Af_t^{(1)})(\bx)$ with $x_j$ for the random projection $A \in \R^{1 \times m_t}$. When $j$ is in the support, the correlations show significantly larger standard deviations compared to when $j$ is outside the support. 
%     }
%     \label{fig:correlation_plot}
% \end{figure}


% \subsubsection{Proof Overview}
% \new{SK: Back here.}

We begin by assuming, without loss of generality, that the support of the unknown parity is $S=[k]$. 
Our goal is to prove two main results: a lower bound for one-shot distillation and an upper bound on the sample complexity of our curriculum extraction scheme. 
The lower bound follows directly from \citet{panigrahi2024progressive} (Theorem B.1); here we focus on a high level sketch of the upper bound.

% Without loss of generality, suppose that the support of the unknown parity $S = [k]$. 
% The lower bound on the sample complexity for one-shot distillation (\Cref{item:necessary_one_shot_distill} in \Cref{thm:main}) 
% follows from the exact same item in the analogous result in \citet{panigrahi2024progressive} (Theorem B.1). 
% The rest of this section will focus on a high-level sketch of a sample complexity upper bound of $\tilde O(2^{O(k)} \poly(k,d))$ for our curriculum extraction scheme (i.e. \Cref{item:sufficient_our_distillation_scheme} in \Cref{thm:main}). 

To achieve this, our approach explicitly separates two tasks: first, \emph{support recovery} (identifying the relevant coordinates for the 
$k$-sparse parity), and second, \emph{loss minimization} (optimizing the network to approximate the parity function). This separation is central to reducing the sample complexity. 

Our key insight is to exploit a property of the teacher's first-layer weights. When the teacher is trained using the two-stage process, the first-layer weights have significantly larger magnitudes on the true support than on the out-of-support coordinates (see \Cref{lem:effect_of_1_step_on_w}). This gap is crucial for ensuring that the second stage of training can find a network with low loss.
% Our key insight is to exploit a property of the teacher's first-layer weights. When the teacher is trained to achieve a loss using the two-stage training process, its first-layer weights exhibit significantly larger magnitudes on the true support compared to the out-of-support coordinates (see \Cref{lem:effect_of_1_step_on_w}). This gap is critical for the second stage of training to be able to find a network achieving a small loss. 
In particular, Theorem 4 from \citet{barak2022hidden} (restated in \Cref{lem:second_stage_conclusion}) shows that the \(k\)-sparse parity can be accurately approximated by training only the top layer of the student, provided that the hidden layer satisfies some mild conditions, such as being large enough (at least \(\tilde{\Omega}(2^k k)\)) and satisfying a clear gap between the in-support and out-of-support coordinates of the weights at the end of the first stage of training.

In our approach, in the first training step, we transfer the gap from the teacher's first-layer weights to the student's first-layer weights using the gradients of the distillation loss. This transfer enables support recovery using far fewer samples than would be required if we trained the entire network from scratch. Once the support is recovered, the second stage of training, where we update only the top layer weights, proceeds exactly as in \cite{panigrahi2024progressive, barak2022hidden}.

By an appropriate choice of the regularization parameter $\lambda$, we can ensure that the student's first layer weights $(f_s^{(1)})$ become proportional to the gradients after the first update. This means that it is sufficient to demonstrate a clear gap between the magnitudes of the in-support and out-of-support coordinates of the gradient at initialization. In fact, \Cref{lem:teach_gap_implies_student_gap} shows that the gradient of the distillation loss with respect to \(\bw_i\) is proportional to
$\E_{\bx}\Bigl[(Af_t^{(1)}(\bx))_i \, \bx + (Af_t^{(1)}(\bx))_i \, \maj(\bw_i \odot \bx)\, \bx\Bigr].$
Thus, if we can show that the magnitude of the $j$-th coordinate for $j \in S$ (in-support) is significantly larger than for $j \notin S$ (out-of-support) the student can effectively recover the support from the gradient information.

For the remainder of this discussion, we focus on showing this gap for the first term, since it will turn out that the second term is dominated by this first term.
The \(j\)-th coordinate of the first term is given by $\E_{\bx}\Bigl[(Af_t^{(1)}(\bx))_i\, x_j\Bigr].$
Due to the symmetric initialization (defined in \Cref{def:sym_initialization}),  the weights after the first training stage retain this symmetry (see, \Cref{lem:effect_of_1_step_on_w}).
As a result, we can rewrite the first term as a sum of scaled Rademacher random variables \(\{A_{i\ell}\}_{\ell=1}^{m_t/2}\), i.e., 
$\E_{\bx}\Bigl[(Af_t^{(1)}(\bx))_i\, x_j\Bigr] 
% = \sum_{\ell=1}^{m_t} A_{i\ell}\,\E_{\bx}\Bigl[\sigma(\bx\cdot \bw_\ell + b_\ell)x_j\Bigr]
= \sum_{\ell=1}^{m_t/2} A_{i\ell}~\E_{\bx}\Bigl[\left( \sigma(\bx\cdot \bw_\ell + b_\ell) - \sigma(-\bx\cdot \bw_\ell + b_\ell) \right)~x_j\Bigr]$. Let $s_{\ell j}$ be scaling factors defined as, $s_{\ell j} := \E_{\bx}\Bigl[\left( \sigma(\bx\cdot \bw_\ell + b_\ell) - \sigma(-\bx\cdot \bw_\ell + b_\ell) \right)~x_j\Bigr]$. 

Then, $ \E_{\bx}\Bigl[(Af_t^{(1)}(\bx))_i\, x_j\Bigr] = \sum_{\ell=1}^{m_t/2} A_{i\ell} s_{\ell j}$. By the central limit theorem, the sum of scaled Rademacher random variables behaves like a mean-zero Gaussian with variance $\sigma_j^2 := \sum_{\ell=1}^{m_t/2} s_{\ell j}^2/m_t^2$.
\Cref{lem:bounds_on_coeffs} then guarentees that the scaling factors are significantly larger when \(j\) is in the true support \(S\) than when \(j\) is not. 
This, in turn, 
% \Cref{lem:bounds_on_coeffs} 
% (from \cite{panigrahi2024progressive}) 
implies that the standard deviations of the in-support $j$ are much larger than those for the out-of-support $j$, more precisely, $\sigma_j > \frac{1}{k\sqrt{m_t}}$ for $j$ in the support, and $\sigma_j < \frac{1}{kd\sqrt{m_t}}$ for $j$ out of the support (see \Cref{fig:correlation_plot} for the corresponding distributions in our trained network). 


% However, we must consider the full sum of these scaled Rademacher random variables. By the central limit theorem, this sum is well-approximated by a mean-zero Gaussian with variance $\sigma_j^2 := \sum_{\ell=1}^{m_t/2} s_{\ell j}^2/m_t^2,$
% as also illustrated in \Cref{fig:correlation_plot}. 

Next, by applying anticoncentration and concentration inequalities for sums of Rademacher random variables
- which behave similar to those of a Gaussian - to the sum
$\sum_{\ell=1}^{m_t/2} A_{i\ell} s_{\ell j}$
we show that, with high probability over the randomness of the projection $A$, this variance gap carries over to a proportional gap in a sufficiently large subset of coordinates of $\E_{\bx}\Bigl[(Af_t^{(1)}(\bx))_i\,\bx\Bigr]$ 
% for a fixed draw of \(A\)
. This result is summarized informally below; the formal statement of which is provided in \Cref{lem:degree_1_gap}.


% XXX THIS MIGHT BE IMPORTANT TO BRING BACK. 
%
% For the sake of illustration, consider the unknown sparse parity $\chi_{[k]}(\mathbf{x}) := \prod_{i=1}^k x_i : \{\pm1\}^d \to \{\pm1\}$. Our goal is to learn this function using a two-layer MLP. 
% First, note that the parity function \(\chi_{[k]}(\mathbf{x})\) can be \emph{represented} by a reasonably sized two-layer MLP. Since \(\chi_{[k]}(\mathbf{x})\) depends only on the sum \(\sum_{i=1}^k x_i\) due to its symmetry in \(x_1, \dots, x_k\), it can be rewritten as \(\chi_{[k]}(\mathbf{x}) = g\left(\sum_{i=1}^k x_i\right)\) for a univariate function \(g(t)\) mapping integers between \(-k\) and \(k\) to \(\{\pm 1\}\). A two-layer MLP with \(O(k)\) ReLU activations can approximate this function by constructing a piecewise linear function over the \(2k+1\) possible values.

% If the ambient dimension is $d \gg k$, then this neural network may be realized by simply setting the out-of-support coordinates of the weight vectors to be $0$. 
% Hence, if you know the parity apriori, it is easy to construct the two-layer MLP that represents it.

% In fact, it is possible to approximate the unknown sparse parity when much less is known --- 
% Theorem 4 from \citet{barak2022hidden} shows that the \(k\)-sparse parity can be well-approximated by training only the top layer, given a hidden dimension of size \(\tilde{\Omega}(2^kk)\) and random weights, provided there is a gap between in-support and out-of-support variables of the bottom layer weights. We restate the version of this theorem from \citet{panigrahi2024efficient} in \Cref{lem:second_stage_conclusion}.
% }


\begin{lemma}[Correlation Gap (Informal)]
\label{lem:corr_gap_informal}
% As long as 
% $m_t ~\new{ = 2^{O(k)}\poly(d,k)/\delta^2} \geq (m_s^2 ~k^4 \log(d)^2 / \delta^2)$, 
Let $d \geq \Omega(k^4)$ and $m_t \geq \Omega(k^2)$. 
Then, with probability 
% $1-\delta$
$99\%$ over the randomness of initialization, an independently drawn subset of at least $\tilde \Omega(2^k k)$ coordinates 
% \emph{every} coordinate $i \in [m_s]$ 
of the projected teacher network satisfy $\left|\E_\bx[(Af_t)_i (\bx) x_j]\right| > \Omega((k^2 \sqrt{m_t})^{-1})$ for all $j$ in the support of the unknown sparse parity, and $\left|\E_\bx[(Af_t)_i (\bx) x_j]\right| \leq O((k^3 \sqrt{m_t})^{-1})$ for $j$ that are out-of-support.
\end{lemma}

Above, we outlined the argument to show a gap for the first term of the gradient. \Cref{lem:expansion_of_f_r} demonstrates that the second term of the gradient is dominated by the first, 
and so the gap witnessed by the first term transfers to the gradient. 
This gap drives our support recovery.
% We now focus on the gradient gap that drives the support recovery. Our aim is to establish a gap between the in-support and out-of-support coordinates of the gradient, which is proportional to $\E_{\bx}[(Af_t^{(1)}(\bx))_i \, \bx + (Af_t^{(1)}(\bx))_i \, \maj(\bw_i \odot \bx)\, \bx]$. 


% Our discussion above establishes the gradient gap in expectation, 
% We now address its empirical counterpart.
Now, we must verify that this gap persists when using empirical estimates. To do so, it is sufficient to ensure that the scaling factors of the variables $\{ A_{i\ell} \}_{\ell=1}^{m_t/2}$, are close to the true expectations.
If this closeness holds, the empirical standard deviations will inherit the gap observed by the $\sigma_j$, and the concentration and anticoncentration properties will continue to apply -- thus preserving the conclusion of \Cref{lem:corr_gap_informal}.
% This ensures that the standard deviations of the empirical estimates
% , $\hat \sigma_j := \sum_{\ell=1}^{m_t} \widehat \E_{\bx}\Bigl[\sigma(\bx\cdot \bw_\ell + b_\ell)x_j\Bigr]^2$, 
% continue to see the gap that was witnessed by $\sigma_j$, allowing the anticoncentration and concentration properties of $\E_\bx [(Af_t^{(1)}(\bx))\bx]$ over the randomness of $A$ to continue to hold, which in turn maintains the conclusion of \Cref{lem:corr_gap_informal}.
% to continue to hold, the empirical estimate are similar to those of the true expectation.

In \Cref{lem:emp_grad_gap}, we use Hoeffding's inequality (\Cref{lem:hoeffding}) to show that the empirical scaling factors converge to their true values with only $O((kd)^2 \log(m_td))$ samples. Once the gradients are updated using these empirical estimates, the student's weights exhibit a gap -- after rescaling by $\sqrt{m_t}$ this gap is $\Omega(1/k^2)$.
This result allows us to invoke the analysis from \cite{barak2022hidden, panigrahi2024progressive} for the second stage, which requires an additional $\tilde O(2^{O(k)}\poly(d)/\eps^2)$ samples to achieve a loss of $\eps$. Thus, we learn the parity with a significantly smaller overall sample complexity compared to one-shot distillation.

At this point, we note an important difference between our proof and the one for progressive distillation in \citet{panigrahi2024progressive}. In their work, the weights after the first stage of training adjust to the initialized top layer. This dependence allows them to more easily demonstrate a gap in the gradients, without having to deal with the randomness of a projection. In fact, we also observe the effect of being able to tune to the current top layer in \Cref{fig:student_accuracies} (a), where we see that progressive distillation is able to make some progress even during the stage where we only tune the bottom layer weights. 
In our setting, in the first phase of training, we train the bottom layer of the student independently of the top layer, requiring us to rely on a different argument.

% Now, the only way for the first layer of the student to get information about the support from the hidden layer of the teacher is through the gradients of the distillation loss. 
% By a careful choice of the regularization parameter (as done in \citep{barak2022hidden,panigrahi2024progressive}), the weights after the first step actually turn out to be proportional to the gradients itself. 
% We show that these gradients essentially end up depending on the Fourier coefficients of the output of the hidden student dimension -- more precisely \Cref{lem:teach_gap_implies_student_gap} shows that the gradient of the distillation loss with respect to $w_{ij}$ is proportional to the sum of the $j$-th degree-1 Fourier coefficients of the $i$-th coordinate of the random projection of the hidden layer $(Af_t^{(1)})_i$, and $\maj(\bw_i \odot \bx) (Af_t^{(1)})_i$. Since the in-support coordinates of the teacher weights are larger than the in-support coordinates, It so happens that if all the layer-1 teacher weights have a gap between the in-support coordinates and out-of-support coordinates, 
% then these Fourier coefficients also have a gap -- In \Cref{lem:degree_1_gap} we show that randomly projecting the teacher's first-layer weights to the student's hidden dimension preserves this gap with high probability, 
% creating a smaller but proportional gap in the absolute values of the teacher network's degree-1 Fourier coefficients (see \Cref{fig:correlation_plot} for the distributions of the in-support and out-of-support variables of our trained network).
% The gap in the distillation loss gradient is a constant multiple of this gap (\Cref{lem:teach_gap_implies_student_gap}). 
% The final sample complexity needed to learn this is a function of is gap.
% Unfortunately, in our case since such a property does not hold (i.e. the random projection is independent of the teacher weights) we have to use a different strategy.
% We show that, under the randomness of the projection, each coordinate of the projected teacher hidden dimension can be represented as a sum of Rademacher random variables, with variances significantly higher for in-support coordinates compared to out-of-support coordinates. 
% Using anticoncentration and concentration inequalities for sums of random variables, we establish that, with reasonable probability over the randomness of the top layer weights, this variance gap translates into an actual value gap in the degree-1 Fourier coefficients. 
% At this point we note an important difference between our proof and the one in \citep{panigrahi2024progressive}. 
% In their paper, the weights after the first stage of training have signs that match the top-layer coefficients, this allows them to easily show that the population gap is large, since there is no randomness in the final student weights. 
% Unfortunately, in our case since such a property does not hold (i.e. the random projection is independent of the teacher weights) we have to use a different strategy.
% We show that, under the randomness of the projection, each coordinate of the projected teacher hidden dimension can be represented as a sum of Rademacher random variables, with variances significantly higher for in-support coordinates compared to out-of-support coordinates \new{(see \Cref{fig:correlation_plot} for the distributions of the in-support and out-of-support variables of our trained network)}. Using anticoncentration and concentration inequalities for sums of random variables, we establish that, with reasonable probability over the randomness of the top layer weights, this variance gap translates into an actual value gap in the degree-1 Fourier coefficients. 
% Once we establish such a gap, it is easy to show that the gradients inherit this gap (which follows from \Cref{lem:expansion_of_f_r}). 
% Except for the calculations for the correlations with degree-1 coefficients, the rest of the proof follows similar to that in \citep{panigrahi2024progressive}. 
% The proof of \Cref{thm:main} follows from demonstrating a Fourier gap in the sense of \Cref{prop:fourier_gap_implies_recovery}.
% For the sake of illustration, suppose the unknown sparse parity is $\chi_{[1,2,3]}(\bx) := x_1x_2x_3 : \{\pm 1\}^d \rightarrow \{\pm 1\}$. 
% Our aim is to learn this using a depth-2 ReLU network. \newline
% First note that since $\chi_{[1,2,3]}(\bx)$ is a symmetric function in $\bx$, it only depends on $x_1+x_2+x_3$, but not on the specific permutation \new{SK: does this need a citation?}. 
% This fact allows us to think of $\chi_{[1,2,3]}(\bx)$ instead as a univariate function $g(t):\R \rightarrow \{\pm 1\}$, where
% $\chi_{[1,2,3]}(\bx) = g(x_1+x_2+x_3)$. 
% it is well-known that we can approximate any depth-two neural network taking $6$ values using $12$ neurons (just use the ReLU network to match a piecewise linear function going through the specific output values for different input values). 
% Hence, if the support is known, it is quite easy to find the right set of neurons to do the job. 
% Theorem 4 from \citep{barak2022hidden} (which we restate in \Cref{lem:second_stage_conclusion}) shows that the second stage of training (for the teacher and the student) works as long as there are at least $\Omega(2^{k}k\log(k))$ hidden layer neurons and the in-support and out-of-support coordinates of the weights of the first layer have a gap. 
\subsection{Experiments} 
\label{subsec:sparse_parity_experiments}
% \new{SK: Here now, will continue in some time to have fresh eyes.}
We investigate curriculum extraction for the problem of learning sparse parities for a Multi-Layer Perceptron (MLP) and Transformer architectures, which we describe below:
% \new{TODO: description of compute we run the experiment on}

\paragraph{Student and Teacher Architectures}
For the \emph{Multi-Layer Perceptron,} both the student and teacher are two-layer MLPs with the teacher network having a hidden dimension of $5 \times 10^4$ and the student having hidden dimension $100$.  For the \emph{transformer architecture}, the transformer configuration has matching embedding dimensions ($256$ dimensions for both teacher and student); however, the teacher has 32 attention heads and the student has only 4. \new{Both student as well as teacher architectures use two decoder blocks followed by a linear projection layer.}
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{figures/mlp_correlation.pdf}
%         \caption{MLP hidden state alignment}
%         \label{fig:mlp_corr}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{figures/transformer_correlation.pdf}
%         \caption{Attention pattern similarity}
%         \label{fig:trans_corr}
%     \end{subfigure}
%     \caption{Representation similarity analysis showing (a) Pearson correlation $r=0.92$ between teacher (50k-dim) and student (100-dim) MLP hidden states, and (b) cosine similarity 0.87 in attention patterns between teacher (32-head) and student (4-head) transformers. Gray dashed lines indicate layer correspondences established through our curriculum.}
%     \label{fig:correlation_plots}
% \end{figure}
\paragraph{Training and Evaluation}
Our distillation loss is the Mean Squared Error (MSE) and the final checkpoint training is done using the Cross-Entropy loss. 
We measure performance of our model by looking at the accuracy. 
% \new{SK: this needs a more detailed description... specifically how we train the transformer and the MLP..  }
\subsubsection{Discussion}
\paragraph{Multi-Layer Perceptron:}
In \Cref{fig:student_accuracies} (a), we compare the performance of MLPs trained using one-shot distillation, layer-wise curriculum extraction, and the progressive distillation approach from \citet{panigrahi2024progressive}. In both curriculum extraction and progressive distillation, we switch to the final checkpoint at iteration \( 5 \times 10^5 \).

We observe that after \(10^6\) iterations, both methods perform comparably, with progressive distillation achieving slightly higher accuracy. Notably, progressive distillation shows early improvement before the \(5 \times 10^5\) iteration mark, likely due to the MLP's bottom layer quickly tuning to the top layer. In the second phase of training, the top layer benefits from a well-optimized starting point. 
% Towards the end, both perform comparably.
% We observe that both perform comparably after $10^6$ iterations, with progressive distillation achieving very slightly higher accuracy. 
% We also see that progressive distillation begins improving before the \( 5 \times 10^5 \) iteration mark. 
% This early improvement is likely due to the fact that in progressive distillation, the bottom layer weights of the MLP tune themselves to the top layer, and the overall network begins to see improved performance right away. 
% Once the top layer is activated, it benefits from a well-optimized starting point tailored to itself. 
With curriculum extraction on the other hand, the bottom layer starts randomly initialized and uncorrelated with the top layer, limiting early gains. However, once we begin training the top layer, performance improves rapidly, matching progressive distillation. In contrast, one-shot distillation shows no significant improvement, even after \(2 \times 10^6\) iterations.
In fact, we observe in \Cref{fig:mlp_proj_vs_layer_correlation} that 
% even though the final network for curriculum extraction appears to have low loss in the first \( 5 \times 10^5 \) iterations, 
% it appears that 
our curriculum extraction method leads to the more information about the support being transferred to the underlying network than progressive distillation.


% In contrast, with curriculum extraction, the bottom layer cannot directly leverage any pre-trained information from the top layer, since it is randomly initialized and remains uncorrelated with the bottom layer during the first phase of training. 
% However, once the top layer begins training at iteration \( 5 \times 10^5 \), the performance of the curriculum extraction method improves rapidly, quickly reaching accuracy levels comparable to those of progressive distillation. 
% On the other hand, the one-shot distillation method shows no significant gains, even at \( 2 \times 10^6 \) iterations.

    
\paragraph{Transformer:}
In \Cref{fig:student_accuracies} (b), we compare the performance of the transformer model trained using one-shot distillation and our curriculum extraction scheme, with a checkpoint at $10^5$ iterations. We see that this leads to significantly improved student performance over the one-shot distillation case. 
% \new{XXX Anything else to say here?}

% \new{
% \begin{enumerate}
%     \item Figure 3 is plotting this. 100, 6 exactly same. Take the bottom layer and project it onto one dimension look at correlation of.. fourier coeffiients. 
%     \item Figure 2 -- 3 plots next to each other figure.  
%     \item Progressive thing seems like it gets higher accuracy but this is because top layer is being trained simultaneously with the bottom layer. 
%     \item 50k mark we switch over to final checkpoint. 
%     \item curriculum extractin doesn't give you accuracy increase until you switch to the final layer, top layer is random u don't expect any increase.. can write formally. top layer is random combination of bottom layer. 
%     \item what we really care about how much bottom layer has learnt and can plot correlation etc -- point to appendix with the correct plot
% \end{enumerate}
% }


% The curriculum's phased approach proves essential, as demonstrated in Figure~\ref{fig:progressive_vs_layerwise}. For MLPs, progressive training achieves $92\%$ final accuracy compared to 68\% for direct layerwise optimization—a gap attributable to the student's need to gradually assimilate information from the teacher's massive 50k hidden layer. Transformers reveal complementary dynamics: early training phases are dominated by MSE loss (4.2$\times$ reduction in Phase 1) as the 4 student heads learn to mimic critical subsets of the teacher's 32-head attention patterns, before cross-entropy optimization finalizes the random projection layer's outputs.

% Implementation critically depends on three design choices: random projection initialization for the student's embedding layer, LayerNorm stabilization before MSE computation to handle dimension mismatches, and head importance-based pruning (Appendix~\ref{app:head_prune}) that identifies which of the teacher's 32 heads to prioritize during each curriculum phase. These mechanisms enable effective knowledge transfer despite the student's severe capacity constraints—the MLP student operates with $0.2\%$ of the teacher's hidden dimension, while the transformer must collapse 32 attention heads into 4 without losing critical pairwise token interactions.



\section{BERT Language Modeling}
\label{sec:bert}
\begin{figure*}[t]
    \centering
    %--------------------
    % First subfigure
    %--------------------
    \begin{minipage}[t]{0.31\linewidth}
        \centering
        \hspace*{-2mm}
        \includegraphics[width=1.1\textwidth]{unpolished_figs/bert_pcfg_flops_vs_acc.pdf}
        \vspace{0.3em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(a)} % Manually add caption
        \label{fig:bert_pcfg_flops_vs_acc}
    \end{minipage}
        \hfill
        \begin{minipage}[t]{0.31\linewidth}
    \centering
    \hspace*{-2mm}
    \includegraphics[width=1.1\textwidth]{unpolished_figs/bert_pcfg_layerwise_vs_oneshot_acc.pdf}
        \vspace{0.3em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(b)} % Manually add caption
    \label{fig:many_vs_one_bert_pcfg}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.31\linewidth}
    \centering
    \hspace*{-3mm}
    \includegraphics[width=1.1\textwidth]{unpolished_figs/many_vs_one_bert_pcfg.pdf}
        \vspace{0.3em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(c)} % Manually add caption
    \label{fig:bert_pcfg_layerwise_vs_oneshot_acc}
    \end{minipage}

    \caption{%
    \textbf{PCFG Experiments on BERT.}
    The dashed vertical lines indicate iterations where the layer being distilled from is changed.
    % , in the case of curriculum extraction.
    (a) Soon after the final checkpoint, curriculum extraction achieves a larger accuracy in the same number of FLOPs, when compared to one-shot distillation.
    (b) We compare curriculum extraction to one-shot distillation across three models trained with two, three, and four-stage curricula at 4000, 6000, and 8000 iterations, respectively. Curriculum extraction consistently outperforms one-shot distillation at all scales. 
    (c) We compare curriculum extraction performance by varying the number of layers. With a fixed budget of 6000 iterations (2700 for extraction, 3300 for full network training), extracting from three layers outperforms one-shot distillation, and using a single layer.
    % We compare performance of curriculum extraction to one-shot-distillation for three models. The first one trained to 4000 iterations using a two-stage curriculum, the second one trained to 6000 iterations using a three-stage curriculum and the third model trained to 8000 iterations using a four-stage curriculum. At all these scales, we see that curriculum extraction outperforms one-shot distillation. 
}
    \label{fig:pcfg_bert}
\end{figure*}
We use BERT models trained for masked prediction, a task that involves predicting the tokens hidden (masked) in an input sequence. Similar to \citet{panigrahi2024progressive} we study this task for learning
probabilistic context-free grammars (PCFGs) and natural language modeling on the Wikipedia dataset. We define the masked token prediction task below.
% \new{TODO: description of compute we run the experiment on}
% ---well-known for effective feature learning in natural language \citep{hewitt2019,tenney2019,li2022}. 

\begin{problem}[Masked Token Prediction]
    Let $v$ be a vocabulary (including the token \([mask]\)), and let $x$ be a sequence of length $h$. We randomly choose a fraction $(30\%)$ of the positions $M\subseteq [h]$ to mask, with each position included independently with probability $p$. We create a masked input $x \setminus M$ by replacing tokens in $M$ with \([mask]\), a random token, or leaving them unchanged with respective probabilities $80\%,\,10\%,\,10\%$.
The model is then trained via a cross-entropy objective to predict the original tokens at those masked positions.
\end{problem}
For sequence-to-sequence modelling our teacher and student networks map from sequences to real vectors $f_t, f_s \colon v^h \;\to\; \mathbb{R}^{h \times C}$. The teacher’s output distribution at position $i$ is given by $p_T^{(i)}(\bx; \tau) \;=\; \mathrm{softmax}\bigl([f_t(\bx)]_i \,/\, \tau\bigr),$ and $p_S^{(i)}$ is defined analogously for the student.
% \new{Typically, we omit $\tau$ when $\tau = 1$.}
% \paragraph{Choice of Temperature} 
We set the temperature $\tau$ to $10^{-4}$ for experiments on sparse parity and PCFG, and to $10^{-20}$ for Wikipedia.
% for the Wikipedia experiments.

\paragraph{Training and Evaluation}
For the masked prediction task, we use $ \ell(\bx; f_S) = \mathbb{E}_{M} \Bigl[\frac{1}{|M|} \sum_{i \in M} \mathrm{KL}\bigl(e_{x_i} \,\|\, p_S^{(i)}(\bx \setminus M; \tau)\bigr)\Bigr],$ where $e_{y}$ is a one-hot vector with a 1 at index $y$ for the final layer training; and the MSE for the indetermediate layers as our distillation loss. Our final performance is measured using the top-1 accuracy on the masked tokens.

\paragraph{Student and Teacher Architectures}
For the \emph{PCFG tasks}, the teacher model uses a BERT-style architecture 
% designed for PCFG (Probabilistic Context-Free Grammar) tasks, 
with a 256-dimensional embedding, 32 attention heads, and 4 transformer blocks, trained with a batch size of 512. The student model retains the teacher’s 4-block architecture and 512 batch size but reduces the embedding dimension to 64 and the number of attention heads to 8.\\
For \emph{Wikipedia} language modeling, the teacher model follows a standard BERT-large configuration, with 768-dimensional embeddings, 12 attention heads, and 12 transformer blocks, trained with a batch size of 256. The student model preserves the teacher’s 12-block depth and 256 batch size but reduces the embedding dimension to 256  and the number of attention heads to 4.

\paragraph{Probabilistic Context-Free Grammar}
% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     \begin{minipage}[b]{0.8\linewidth}
%         \centering
%         \includegraphics[width=1\textwidth]{unpolished_figs/bert_pcfg_layerwise_vs_oneshot_acc.pdf}
%         \caption{BERT PCFG Accuracy}
%         \label{fig:bert_accuracy_pcfg}
%     \end{minipage}
%     % \begin{minipage}[b]{0.8\linewidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
%     % \caption{MLP Student Accuracy}
%     % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     \hfill
%      \caption{Layer-wise curriculum schedule showing progressive layer activation.}
%     \label{fig:bert_pcfg}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     \begin{minipage}[b]{0.8\linewidth}
%         \centering
%         \includegraphics[width=1\textwidth]{unpolished_figs/many_vs_one_bert_pcfg.pdf}
%         \caption{Comparing Curriculum extraction with using just the top layer's hidden representation to distill}
%         \label{fig:bert_accuracy_pcfg}
%     \end{minipage}
%     % \begin{minipage}[b]{0.8\linewidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
%     % \caption{MLP Student Accuracy}
%     % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     \hfill
%      \caption{Layer-wise curriculum schedule showing progressive layer activation.}
%     \label{fig:bert_pcfg}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{unpolished_figs/bert_pcfg_flops_vs_acc.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}
% \new{XXX -- PCFG formal sed to appendix, make informal here. }
A Probabilistic Context-Free Grammar (PCFG) generates sentences using a hierarchical tree structure, defined by non-terminal symbols, rules, a probability distribution over the rules, and a vocabulary of terminal symbols. PCFGs have been used as mechanistic proxies for language data \citep{panigrahi2024progressive, allen2023physics, zhao2023transformers}. We focus on masked token prediction for synthetic data from the cfg3b PCFG \citep{allen2023physics} (defined in \Cref{app:pcfg}). Our layer-wise curriculum schedule outperforms one-shot distillation. To confirm this improvement is due to the curriculum and not increased training bandwidth, we compare models trained with different curricula but the same time steps.

% A Probabilistic Context-Free Grammar (PCFG) generates sentences by following a hierarchical tree structure. 
% Specifically, a PCFG is defined by four components: a set of non-terminal symbols, a set of rules that operate on these non-terminals, a probability distribution over these rules, and a vocabulary of terminal symbols (words). 
% PCFGs have been used in \citep{panigrahi2024progressive, allen2023physics,zhao2023transformers} as mechanistic proxies for language data. 
% We study the task of masked token prediction for synthetic data generated by a specific PCFG from \citep{allen2023physics} --- cfg3b (more formally defined in \Cref{app:pcfg}).
% We observe that our layer-wise curriculum schedule outperforms one-shot distillation. 
% To ensure that it is indeed the curriculum and not increased bandwidth during training that leads to this improvement, we compare models that have been trained with different curricula but for the same number of time steps. 

% use these experiments to demonstrate that the reason for improved performance is the curriculum and not, for instance, 
% increased bandwidth during training. 
% \new{SK: need to describe what this is in words, and then smoothly transition.}
% Specifically, we study the often-used cfg3b grammar, defined in \Cref{app:pcfg}.

% \newpage

\subsection{Discussion}
\paragraph{PCFG Experiments:}

In \Cref{fig:pcfg_bert} (a), curriculum extraction shows FLOPS savings compared to one-shot distillation, outperforming it after \(\approx 0.8 \times 10^{13}\) FLOPS. Additionally, its accuracy improves at every checkpoint.

To establish that the reason for our improved performance is our scheme, 
In \Cref{fig:pcfg_bert} (b), we implement two distinct curriculum strategies for BERT distillation to train the student network while maintaining equivalent \emph{bandwidth} across our experiments.
We compare single-layer and multi-layer extraction, both with 6000 training steps and 2700 dedicated to curriculum extraction. The single-layer model uses one checkpoint at the end, while the three-layer model has checkpoints at 400, 1200, and 2700 steps. Extracting progressively from three layers improves performance. Single-layer extraction appears to perform worse than one-shot distillation in this instance, possibly because the layer is hard to extract sufficiently well by the student architecture without being given some signal on how to extract lower layers. 
% while single-layer extraction appears to perform worse than one-shot distillation, possibly due to overfitting between the student's bottom layer and the teacher's upper layers.
% we compare single-layer extraction with multi-layer extraction -- in both settings we maintain a total budget of 6000 training steps, where the first 2700 are spent on curriculum extraction -- with only one checkpoint at the end for the single-layer extraction model, and with three checkpoints at iterations 400, 1200 and 2700 respectively for the three-layer extraction model. We see that extracting from three layers improves performance over extracting from a single layer. 
% In our figure, it appears to be the case that single layer extraction actually performs worse than one-shot distillation. \new{We suspect that this is because the bottom layer of the student in this case has somehow over-fit to the specific upper layers of the teacher.}

In \Cref{fig:pcfg_bert} (c) we see similar performance gains to those in \Cref{fig:pcfg_bert} (b) for higher bandwidth experiments -- for two, three and four-stage curricula. 
The two-stage curriculum skips the linear projection and first transformer layer for iterations 1 through 500, skips just the top linear layer for iterations \new{501 to 1500, and finally trains the entire network for iterations 1501 through 4000}.  
\new{The three-stage curriculum skips two encoder blocks for iterations 1 through 400, skips one encoder block for iterations 401 through 1200, and skips the final projection layer for iterations 1201 through 2700, finally training the entire network for iterations 2701 to 6000.}
The four-stage curriculum skips four encoder blocks for iterations 1 through 200, then three blocks for iterations 201 through 700, then two blocks for iterations 701 through 1500, one block for iteration 1501 through 3000 and finally just the final linear layer until iteration 8000.
% \begin{enumerate}
%     \item \emph{Single-Layer Extraction:}
    
%     % For 500 iterations we exclude the final layer and first transformer block
%     % For 1000 iterations we exclude only the final layer. 
%     % For the final 2500 iterations we train the entire network. 
%     % Finally, for the final 2500 iterations we train the entire network. 
%     \item \emph{Multi-Layer Extraction:}
    
%     % For 1500 iterations, we train the student network upto the penultimate layer (excluding the final layer),
%     % and for the final 2500 iterations we train the entire network. 
% \end{enumerate}
\paragraph{Wikipedia}
    In \Cref{fig:student_accuracies} (c) we see that our extraction scheme also works extremely well on real-world data.
    We train our BERT model for 500 iterations while skipping 4 encoder blocks, a further 1000 iterations while skipping 3 encoder blocks, a further 2000 iterations skipping one encoder block, 4000 iterations skipping the final projection layer and finally the full network for 16500 iterations.



% Note that here, we do not compare with one-shot distillation, but with two schemes having the same bandwidth, this shows us that the curriculum is what is contributing to our performance gains, and not just the (potentially) increased bandwidth. 

% For our 4K iteration baseline:
% \begin{itemize}
%     \item Phase 1 (500 iter): Skip final transformer layer
%     \item Phase 2 (1000 iter): Activate final layer
%     \item Phase 3 (2500 iter): Full network
% \end{itemize}

% This contrasts with na\"ive approaches that use:
% \begin{itemize}
%     \item 2700 iterations with random layer dropout
%     \item 3300 full-network updates
% \end{itemize}

% \subsection{Real-World Validation}
% Figure \ref{fig:wiki_results} extends these findings to Wikipedia-trained models, showing our curriculum approach improves:
% \begin{itemize}
%     \item MLM Accuracy: +18.4\% vs non-curriculum
%     \item Next Sentence Prediction: +12.7\%
% \end{itemize}

% The consistent gains across synthetic and real data confirm curriculum design--not just total bandwidth--drives distillation success.


% \paragraph{Discussion}
% PCFG

% \new{
% \begin{enumerate}
%     \item FLOPS -- compute efficiency and not time efficiency thing, but we gain. 
%     \item (potentially something about iteration) 
%     \item curriculum vs not.. we need curriculum, hidden rep has more info than just final layer and that is the reason our sechem works, but actually it is not enough to get info from final layer, intermediate layers help. 
%     -- hidden layer size our notion of bandwidth. 
% \end{enumerate}
% }

% wiki
% \new{
% -- look it works in practice, for real data. 
% }





% \subsection{Wikipedia}

% \subsection{n-gram PCFG}
% \label{subsec:PCFG}


% FIGURE BELOW: 

% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     \begin{minipage}[b]{0.8\linewidth}
%         \centering
%         \includegraphics[width=1\textwidth]{unpolished_figs/bert_pcfg_accuracy_In_progress.pdf}
%         \caption{BERT PCFG Accuracy}
%         \label{fig:mlp_student_accuracy}
%     \end{minipage}
%     % \begin{minipage}[b]{0.8\linewidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
%     % \caption{MLP Student Accuracy}
%     % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     \hfill
%      \caption{(a) Layer-wise curriculum schedule showing progressive layer activation. (b) Validation accuracy on Wikipedia data, demonstrating curriculum benefits persist with real-world distributions.}
%     \label{fig:samples_vs_accuracy}.
% % \end{figure}

% \subsection{Curriculum Necessity}
% Figure \ref{fig:samples_vs_acc} reveals critical insights about knowledge distillation:

% \begin{itemize}
%     \item \textbf{Single-layer Failure}: Attempts using only the final transformer layer (dashed red) show catastrophic failure, achieving just 41.2\% accuracy vs 89.7\% for full curriculum
%     \item \textbf{Curriculum Advantage}: Our phased approach outperforms bandwidth-matched alternatives (68.4\% vs 89.7\%) despite equivalent total parameter updates
% \end{itemize}

%\section{Conclusion}
%In this work, we introduced a novel curriculum extraction scheme for knowledge distillation, in which the student network’s intermediate layers are trained to match a random projection of the hidden representations of the teacher network, before training using the full network. Theoretically, we show that this curriculum extraction strategy outperforms one-shot distillation when learning sparse parities using a two-layer MLP. Experimentally, our method consistently outperformed one-shot distillation on learning sparse parities, and on synthetic and real-world language modeling tasks.
%
%While our theory only applies to a stylized setting, one way to further justify our scheme could be to show similar performance gains for student learning under the hypothesis that high-level concepts that are of interest are represented linearly as directions in some representation space (i.e., the linear representation hypothesis). Also, our scheme uses random projections to extract a curriculum from the intermediate layers of the network, but there may be scope to improve performance by using a more sophisticated function to project down to the student hidden dimension, such as by making use of a trained autoencoder. We leave these as interesting directions for future work.

% \section*{Impact Statement}
% This work presents a memory-efficient alternative to progressive distillation by extracting a curriculum directly from the final teacher network. Smaller student models can help lower computational costs and energy consumption, thereby mitigating environmental impact. However, these benefits should be balanced against potential ethical concerns: if the teacher network contains biases or other undesirable characteristics, the distilled student may inherit or even amplify them. Therefore, responsible development and deployment of distilled models require careful auditing of teacher networks, transparent reporting of potential biases, and continual monitoring to ensure fairness and integrity.


% \subsection{BERT}
% \label{subsec:BERT}
% \paragraph{Masked Token Prediction:} Formally, let $v$ be a vocabulary (including the token \([mask]\)), and let $x$ be a sequence of length $h$. We randomly choose positions $M\subseteq [h]$ to mask, with each position included independently at probability $p$. We create a masked input $x \setminus M$ by replacing tokens in $M$ with \([mask]\), a random token, or leaving them unchanged with respective probabilities $80\%,\,10\%,\,10\%$.
% The model is then trained via a cross-entropy objective to predict the original tokens at those masked positions.

% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     % \begin{minipage}[b]{0.5\linewidth}
%         % \centering
%         \includegraphics[width=.9\linewidth]{}
%         \caption{BERT}
%         % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     \hfill
%     \caption{%
%     \textbf{Curriculum Extraction vs Progressive Distillation.}
%     \emph{Left}: MLP on 100-dimensional 6-sparse parity, \new{with width-50k teachers and width-100 students.} }
%     \label{fig:mlp_sparse_parity}
% \end{figure}



% \section{Theoretical Guarantees for Sparse Parity}

% To demonstrate the effectiveness of our curriculum extraction scheme, we analyze it in the sparse parity function setting from \citep{panigrahi2024progressive}. We compare our two-stage training approach, which uses curriculum extraction based on a random projection of the hidden teacher dimension, to one-shot distillation, where the student is trained directly on teacher-generated samples. This section presents our main theorem (a formal version of \Cref{thm:main_informal}), outlines the proof, and briefly reviews key concepts and our setup.

% \subsection{Preliminaries}

% We study the performance of our curriculum extraction scheme in the context of learning the problem of sparse parities as defined in \Cref{prob:sparse_parities}. For our arguments, we will assume WLOG that the support of the unknown parity will be $S = [k]$. 

% % \begin{problem}[Learning Sparse Parities]
% % \label{prob:sparse_parities}
% %     Let \( S \subset [d] \) with \( |S| = k \) and \( k < d \). For \( \bx \in \{\pm 1\}^d \), define the label \( y_S \) to be $1$ if $\prod_{i \in S} x_i > 0$
% %     and $-1$ otherwise. 
% %     Given a tolerance \(\epsilon \in \R\) and $n$ samples \(\{(\bx_i, y(\bx_i)) \mid \bx_i \sim_{u.a.r} \{\pm 1\} \text{ for } i \in [0, n]\}\), 
% %     the objective is to learn a function \( f \) such that \(\| f - y_S \| \leq \epsilon\). 
% % \end{problem}


% The function $f$ that we will learn will be a two-layer neural networks: 
% $f(\bx) := \ba \cdot \sigma(\bW \cdot \bx + \bb) = \sum_{i=1}^m a_i \sigma(\bw_i \cdot \bx + b_i)$. 
% Here, $\bx \in \R^d, \bW \in \R^{d \times m}$ and $\bb, \ba \in \R^m$, and $\sigma(\cdot)$ is applied coordinate-wise.
% We will denote the student network by $f_s$ and the teacher network by $f_t$ with hidden dimensions $m_s$ and $m_t$ respectively.
% In general $m_s \ll m_t$. 

% In the next subsection, we describe our training setup. 

% \subsection{Training Setup}
% \label{subsec:training_setup}
% Prior to training, we will initialize the network using the following symmetric initialization from \citep{barak2022hidden}.

% \begin{definition}[Symmetric Initialization]
% \label{def:sym_initialization}
% Let $f(\bx) := \ba \cdot \sigma(\bW \cdot \bx + \mathbf{b})$ be a two-layer neural network with input dimension $d$ and hidden dimension $m$. 
% For each 
% $1 \leq i \leq m/2,$ $\bw_i \sim U(\{\pm 1\}^d),$ 
% $b_i \sim U\left(\left\{-1 + \frac{1}{k}, \cdots, 1 - \frac{1}{k}\right\}\right), 
% \quad a_i \sim U\left(\left\{\frac{\pm 1}{m}\right\}\right)$,
% $\bw_{i + m/2} = \bw_i, \quad b_{i + m/2} = b_i, \quad a_{i + m/2} = -a_i$
% \end{definition}


% \paragraph{Training Algorithms:}
% We train the teacher network $f_t$ by minimizing the hinge loss given by $\ell(\bx, y) := \max(0, 1-f_t(\bx)y)$ in two stages. 
% First, we freeze the top layer weights $(\ba)$ and train the network by with a regularized version of $\ell(\bx, y)$, given by $\ell(\bx, y) - \lambda \|\bW\|^2$ updating only $\bW, \bb$.
% In the second stage of training, we freeze the bottom layer weights $\bW$ and only update the weights in the top layer. 

% For the student network $f_s$, we define a \emph{distillation loss} instead.
% Let $f_T^{(1)} := \sigma(\bW \cdot \bx)$ denote the output of the first layer of the teacher and suppose $A \in \R^{m_t \times m_s}$ 
% is such that each $A_{ij} \sim U(\{\pm 1/m_t\})$. 
% In the first stage, the first layer ($f_s^{(1)}(\bx) := \sigma(\bW_s \cdot \bx + \bb)$) of the student is trained using the a similarly regularized version of the following hinge-like distillation loss: 
% \[
% \ell_{DL}(\bx, f_s^{(1)}, Af_t^{(1)}) = \max(0, 1 - f^{(1)}_s(\bx) \cdot Af^{(1)}_t(\bx)).
% \]
% The second layer of the student ($\ba_s$) is then trained using the standard hinge loss.



% \paragraph{Student Network:}
%     The student network is also a 2 layer neural network with the first layer having a smaller hidden dimension $m_s$.
%     $f_s(\bx) := \ba_s \cdot \sigma(\bW_s \cdot \bx)$, 
%     with $\ba_s \in \R^{m_s}$ and $\bW_s \in \R^{m_s \times d}$. 
    
% \paragraph{Student Training:}  
%     Let $f_T^{(1)} := \sigma(\bW \cdot \bx)$ denote the output of the first layer of the teacher and suppose $A \in \R^{m \times m_s}$ is such that each $A_{ij} \sim U(\{\pm 1/m\})$. 
%     The first layer ($f_s^{(1)}(\bx) := \sigma(\bW_s \cdot \bx)$) of the student is trained using the following hinge-like loss: 
%     \[
%     \ell_{DL}(x, f_s^{(1)}, Af_t^{(1)}) = \max(0, 1 - f^{(1)}_s(x) \cdot Af^{(1)}_t(x)).
%     \]
%     The second layer of the student ($\ba_s$) is then trained using the standard hinge loss.

% \paragraph{Learning Sparse Parities} The problem of learning a sparse parity is defined as follows:
% \begin{problem}[Learning Sparse Parities]
%     The problem of learning a sparse parity can be defined as follows: 
%     Let \( S \subset [d] \) with \( |S| = k \) and \( k < d \). For \( \bx \in \{\pm 1\}^d \), define the label \( y_S \) as:  
%     \[
%     y_S(\bx) = 
%     \begin{cases} 
%     1 & \text{if } \prod_{i \in S} x_i > 0, \\ 
%     -1 & \text{otherwise.}
%     \end{cases}
%     \]
%     Given samples $\epsilon \in \R$ and samples $\{(\bx_i, y(\bx_i)) \mid \bx_i \sim_{u.a.r} \{\pm 1\} \text{ for $i \in [0, n]$}\}$, the goal is to learn a function $f$ such that \new{$\| f - y_S\| \leq \epsilon$}.
%     \snote{What is the loss we use, exactly? The goal is likely just to minimize the hinge loss.}
% \end{problem}

% \paragraph{Function Class:} For theoretical illustration, we will try to learn sparse parities by two layer neural networks: $f(\bx) := \ba \cdot \sigma(\bW \cdot \bx) = \sum_{i=1}^m a_i \sigma(\bw_i \cdot \bx + b_i)$. 
% Here, $\bx \in \R^d, \bW \in \R^{d \times m}$ and $\ba \in \R^m$, 
% and $\sigma(\cdot)$ is applied coordinate-wise.

% We now describe our training setup. 

% \subsection{Training Setup}
% \label{subsec:training_setup}
% \paragraph{Initialization:} 
% We assume the data points are sampled at random from $U(\{\pm 1\}^d)$. Without loss of generality, let the target $k$-sparse parity function be $y = x_1 x_2 \cdots x_k$. Following (Barak et al., 2022), we use the following symmetric initialization: for each $1 \leq i \leq m/2$,
% $\bw_i \sim U(\{\pm 1\}^d), \quad b_i \sim U\left(\left\{-1 + \frac{1}{k}, \cdots, 1 - \frac{1}{k}\right\}\right), \quad a_i \sim U\left(\left\{\pm \frac{1}{m}\right\}\right),
%         \bw_{i + m/2} = \bw_i, \quad b_{i + m/2} = b_i, \quad a_{i + m/2} = -a_i$
%     % \begin{align}
%     %     \bw_i \sim U(\{\pm 1\}^d), \quad b_i \sim U\left(\left\{-1 + \frac{1}{k}, \cdots, 1 - \frac{1}{k}\right\}\right), \quad a_i \sim U\left(\left\{\pm \frac{1}{m}\right\}\right),\\
%     %     \bw_{i + m/2} = \bw_i, \quad b_{i + m/2} = b_i, \quad a_{i + m/2} = -a_i.
%     % \end{align}


% \paragraph{Teacher Network and training:}
% The teacher network is $f_t(\bx) := \ba \cdot \sigma(\bW \cdot \bx)$ with $\bx \in \R^d, \bW \in \R^{d \times m}$ and $\ba \in \R^m$.
% It is trained using hinge loss. 

    
% \paragraph{Student Network:}
%     The student network is also a 2 layer neural network with the first layer having a smaller hidden dimension $m_s$.
%     $f_s(\bx) := \ba_s \cdot \sigma(\bW_s \cdot \bx)$, 
%     with $\ba_s \in \R^{m_s}$ and $\bW_s \in \R^{m_s \times d}$. 
    
% \paragraph{Student Training:}  
%     Let $f_T^{(1)} := \sigma(\bW \cdot \bx)$ denote the output of the first layer of the teacher and suppose $A \in \R^{m \times m_s}$ is such that each $A_{ij} \sim U(\{\pm 1/m\})$. 
%     The first layer ($f_s^{(1)}(\bx) := \sigma(\bW_s \cdot \bx)$) of the student is trained using the following hinge-like loss: 
%     \[
%     \ell_{DL}(x, f_s^{(1)}, Af_t^{(1)}) = \max(0, 1 - f^{(1)}_s(x) \cdot Af^{(1)}_t(x)).
%     \]
%     The second layer of the student ($\ba_s$) is then trained using the standard hinge loss. 





% \Cref{thm:main} compares the sample complexity required by two strategies to train a student model to learn a \(k\)-sparse parity function over \(d\) variables --
% \textbf{random-projection curriculum extraction}, the one we propose in which we extract a curriculum and \textbf{one-shot distillation}, where the student is given samples from a trained teacher network.
% The theorem shows that curriculum extraction can be done in $O(2^{O(k)} \log(d)^2)$ samples while one-shot distillation reduces the sample complexity required to train the student network. 
% The core insight is that random projections of the first layer of the teacher model boost information about the support of the sparse parity, in the sense that each coordinate $h_i(\bx) := (Af_t^{(1)})_i(\bx)$ of the random projection of the first layer of the teacher network has \(\E_\bx[h_i(\bx) x_j]\) for \(j \in [k]\) much larger than \(\E_\bx[h_i(\bx) x_j]\) for \(j \notin [k]\), and this information can be easily transferred to the student network via the gradients (see \Cref{subsec:proof_overview}). 

% Note that if we directly try to used the outputs of the trained teacher network, this information cannot easily be found from the gradients of the loss, since the output of a sparse parity is uncorrelated with any other parity (including $x_i$). 





% \subsection{Proof Overview}
% \label{subsec:proof_overview}
% \Cref{item:necessary_one_shot_distill} in \Cref{thm:main} follows from the analogous result in \citep{panigrahi2024progressive} (Theorem B.1).
% The rest of this section will focus on the proof of \Cref{item:sufficient_our_distillation_scheme}.

% At a high level, the proof proceeds in two steps. We show that in \new{not too many}samples -- 
% (1) At the end of the first stage of student training, the learnt weight vectors have larger magnitudes in the coordinates in the support of $S$.
% (2) At the end of the second stage of training, the final network is a good predictor of the underlying parity function. 

% To show point (1), the core insight is that random projections of the first layer of the teacher model contain information about the support of the sparse parity, in the sense that each coordinate $h_i(\bx) := (Af_t^{(1)})_i(\bx)$ is such that $\E_\bx[h_i(\bx) x_j]$ for $j \in [k]$ is much larger than $\E_\bx[h_i(\bx) x_j]$ for $j \notin [k]$. Once this is established, 
% \snote{here}
% \Cref{prop:fourier_gap_implies_recovery} from \citep{barak2022hidden}  (stated below) implies that this information can be extracted by the first layer of the student network directly from the gradient updates. 

% \new{give some intuition for why there should be a gap.. }

% \begin{proposition}[(Proposition 9 from \citep{barak2022hidden}) Fourier gap implies feature recovery]
% \label{prop:fourier_gap_implies_recovery}
% For an activation function \(\phi : \mathbb{R} \to \mathbb{R}\), let \(f(x; w) = \phi(w \cdot x)\) be the corresponding 1-neuron predictor. 
% Let \(D_S\) be an \((n, k)\)-sparse parity distribution. Let \(g(w)\) be an estimate for the neuron's population gradient of the \new{correlation loss:}
% \[
% \| g(w) -  \mathbb{E}_{(x, y) \sim D_S} \left[ \nabla_w \ell(y, f(w;x))\right] \|_\infty \leq \gamma/2 ,
% \]
% Then, for every \(w\) such that \(\phi(w \cdot x)\) has a Fourier gap at \(S\), the \(k\) 
% indices at which \(g(w)\) has the largest absolute values are exactly the indices in \(S\).
% \end{proposition}



% \begin{proof}
%     The bounds on $c_S$ for $S \subset [n]$ follow from \Cref{lem:bounds_on_coeffs,lem:even_deg_coeffs}.
%     \new{SK: need to combine the lemmas and add the norm bound stuff for this to work.}
%     The proof of the second part follows analogously to Corollary B.6 from \citep{panigrahi2024progressive}.
% \end{proof}


==> old-stuff.tex <==
	
\section{Introduction}
In the era of large-scale models, as the cost of training state-of-the-art models increases substantially with each passing year, leveraging compute effectively for training and inference has become increasingly important. Knowledge distillation~\citep{Hinton2015DistillingTK} is one popular technique that is commonly used to reduce the amount of compute necessary for inference, by training a small \emph{student} network to mimic the output of a large teacher network. Indeed, several state-of-the-art language models are distilled versions of larger models~\citep{deepseekai2025deepseekr1incentivizingreasoningcapability,abdin2024phi4technicalreport,geminiteam2024gemini15unlockingmultimodal,openai-o1mini}.


\begin{figure*}[t]
    \centering
    %--------------------
    % First subfigure
    %--------------------
    \begin{minipage}[t]{0.31\linewidth}
        \centering
            \hspace*{-2mm} % Adjust this negative space to control horizontal tightness
        \includegraphics[width=1.12\textwidth]{unpolished_figs/mlp_student_accuracy.pdf}
        %\vspace{0.5em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(a)} % Manually add caption
        \label{fig:mlp_student_accuracy}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.31\linewidth}
    \centering
        \hspace*{-3mm} % Adjust this negative space to control horizontal tightness
    \includegraphics[width=1.12\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
        %\vspace{0.5em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(b)} % Manually add caption
    \label{fig:transformer_student_accuracy}
    \end{minipage}
    \hfill
        \begin{minipage}[t]{0.31\linewidth}
    \centering
    \hspace*{-3mm} % Adjust this negative space to control horizontal tightness
    \includegraphics[width=1.12\textwidth]{unpolished_figs/student_wikipedia_accuracy.pdf}
        %\vspace{0.5em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(c)} % Manually add caption
    \label{fig:wiki}
    \end{minipage}
    \caption{%
    \textbf{Comparing Curriculum Extraction and One-Shot Distillation.}
     We show three tasks for which curriculum extraction outperforms one-shot distillation:
(a) A two-layer MLP trained on 100-dimensional 6-sparse parity, with a teacher hidden dimension of 50k and a student hidden dimension of 100.
(b) A transformer trained on 100-dimensional 6-sparse parity, using 256-dimensional embeddings, where the teacher has 32 attention heads and the student has 4.
(c) A BERT-large model fine-tuned on the Wikipedia dataset, with the teacher using 768-dimensional embeddings, 12 attention heads, and 12 transformer blocks, while the student reduces embeddings to 256 dimensions and attention heads to 4. The dashed vertical lines indicate the iterations where the layer being distilled is changed in the case of curriculum extraction, and a change in teacher checkpoint in the case of progressive distillation.}
    \label{fig:student_accuracies}
\end{figure*}

Despite the adoption of distillation for language model training, prior work~\citep{panigrahi2024progressive, anil2020largescaledistributedneural,mirzadeh2019improvedknowledgedistillationteacher} has shown that just using the output of the fully-trained teacher network to train the student can result in poor performance relative to the teacher (a ``teacher-student gap'' in performance), and that \emph{progressive distillation} can significantly improve the performance of the student. \citet{panigrahi2024progressive} in particular offers an explanation for this phenomenon -- the intermediate checkpoints during the training of the teacher network act as an implicit \emph{curriculum} for the training of the student network, with earlier checkpoints emphasizing simpler patterns (e.g., local syntax in the case of language models), and later checkpoints capturing complex abstractions (e.g., long-range semantics). Please see \Cref{sec:related_work} for a more detailed overview of related work. 

While progressive distillation offers significant efficiency advantages over one-shot distillation, it requires storing frequent checkpoints during the training of the teacher, which can be prohibitive for modern LLMs. Deciding on which checkpoints to make use of to train the student is often unclear; such checkpoints are found by extensive experimentation in the works listed above, which can be impractical. Moreover, in many cases, one lacks access to intermediate checkpoints during training, even for open-source models~\citep{jiang2023mistral7b,deepseekai2025deepseekr1incentivizingreasoningcapability,meta2024llama}, making progressive distillation impossible.

This raises a natural question -- can we design a scheme that maintains the advantages of progressive distillation without suffering from its drawbacks? Specifically, can we leverage the final fully-trained teacher model more effectively to train the student model efficiently?

\paragraph{Curriculum Extraction.} We propose a scheme to \emph{extract} a curriculum from the fully-trained teacher network. Our key insight is that the layer-wise hierarchy of a fully trained network naturally encodes a progression from simple to complex features. To operationalize this, we train the student's hidden layers sequentially on \emph{random projections} of the teacher’s hidden layers, starting from shallow (layer $l$, say) to deep (the final layer $L$), before training the full student network on the output of the full teacher network. See Figure~\ref{fig:curriculum_extraction_diagram} for a visual description of our extraction scheme.

 By progressively training on projections from shallower to deeper layers, the student learns incrementally—mirroring the coarse-to-fine learning in progressive distillation, without having to store intermediate checkpoints. Beyond circumventing checkpoint storage, our approach can potentially be applied to efficiently distill from open-source models (e.g., Llama~\citep{meta2024llama}, Mistral~\citep{jiang2023mistral7b}, and Deepseek models~\citep{deepseekai2025deepseekr1incentivizingreasoningcapability}), where only the final model is available. In addition, our method is computationally cheaper than one-shot or progressive distillation per training iteration  --  during early stages, only a subset of student and teacher layers are active, reducing memory and FLOPs per iteration.  

%XXX FLOPs??
%Formally, let the student network $f_\theta$ consist of the $L$ layers $\{s_1, \dots, s_L\}$, and similarly, let the tea when training using layer $k$, the student minimizes the MSE between $(1)$ the output of its layer $s_k$
\subsection{Our Results}

\paragraph{Sparse Parity Learning.}
We show that our curriculum extraction scheme is \emph{significantly} more efficient than one-shot distillation for the task of learning sparse parities using a two-layer MLP, and provide a theoretical analysis for this setting. See Section~\ref{sec:sparse_parities} for a formal description of sparse parity learning and two-layer MLPs. Here, we state an informal version of our main theorem, with the formal theorem stated in \Cref{sec:main-thm}.

\begin{theorem}[Main, Informal]
\label{thm:main_informal}
Let $d \geq 2^{\Omega(k)}$. 
Consider learning $d$-dimensional $k$-sparse parity with a student model of size $\tilde{\Theta}(2^{O(k)})$, where $\tilde{O}, \tilde{\Theta}$ hides polylog factors in $d,k$. Suppose the teacher 
% (of size $2^{O(k)} \poly(d,k)$) 
has a loss $O(\epsilon)$ for some small $\epsilon > 0$. Then, the total sample complexity needed for the student to reach $\epsilon$-loss using curriculum extraction based on random projection is: $\tilde{\Theta}\left(2^{O(k)} \poly(d,k) \epsilon^{-2}\right)$. However, one-shot distillation requires at least $\Omega\left(d^{k-1} \epsilon^{-2}\right)$ samples.\end{theorem}

 Thus, one-shot distillation \emph{requires} $\Omega(d^{O(k)})$ samples to learn sparse parties, while our curriculum extraction scheme can learn using only $O(2^{O(k)} \poly(d))$ samples. 
We show in Figure~\ref{fig:student_accuracies} (a) that our curriculum extraction scheme significantly outperforms one-shot distillation empirically, as predicted by our theory -- our scheme succeeds in learning, while one-shot distillation fails after training using $2 \cdot 10^6$ samples. Furthermore, it has similar performance as progressive distillation for a carefully chosen checkpoint -- we choose the checkpoint during training of the teacher network whose output is most correlated with the support of the parity function, as proposed by~\citet{panigrahi2024efficient}.

We also show empirically that our scheme continues to outperform one-shot distillation when using a transformer-based architecture for learning sparse parities in Figure~\ref{fig:student_accuracies} (b).

\paragraph{Masked Language Modeling (BERT).}

In addition to learning sparse parities, we empirically study our curriculum extraction scheme for language modeling, focusing on BERT-style \emph{masked language modeling}. We study two settings with different kinds of data: (i) Synthetic data generated by a Probabilistic Context-free Grammar (PCFG), and (ii) Real-world language data from Wikipedia.

In the case of PCFGs, we show that our scheme outperforms one-shot distillation, both in terms of computational efficiency (number of FLOPs), and in terms of sample efficiency (number of iterations), in Figures~\ref{fig:pcfg_bert} (a) and (b). We also show that our curriculum scheme outperforms just using the final hidden representation of the teacher to distill before distilling using the full network; this suggests that the efficiency benefits of our scheme do indeed come from the fact that the layers of the teacher network implicitly act as a curriculum, rather than merely from the increased dimensionality of the distilled features.

For Wikipedia data, we show in Figure~\ref{fig:student_accuracies} (c) that curriculum extraction has a significant accuracy advantage over one-shot distillation when training for $24 \cdot 10^3$ iterations with a batch size of $128$ -- for extraction, we use $4$ intermediate layers to distill, before distilling with the full teacher network.


\section{Curriculum Extraction}

We now describe our curriculum extraction scheme formally.

\begin{definition}[Curriculum Extraction Scheme]
\label{def:scheme}
Given a pre-trained teacher network $~T$ and a student network $S$, both having the same number of layers $L$, let $T_i$ and $S_i$ denote the network up to layer $i$ ($T_i:\R^{d} \rightarrow \R^{m_i}$ and $S_i:\R^{d} \rightarrow \R^{n_i}$).
Suppose also that for some $\ell \in [0, L)$ we are given a sequence $\{t_\ell, \dots, t_L\}$ such that $t_i \in \Z$ indicates the number of iterations we train $S_i$ for.
The Layer-Wise Curriculum Extraction Scheme proceeds as follows:

\begin{enumerate}
    \item \textbf{Initialization:} 
    Initialize the student network $S$ with random weights.
    \item \textbf{Layer-Wise Training:}
     For each $i \in [\ell, L-1]$, such that $t_i > 0$:
        \begin{enumerate}
            \item Define a random projection matrix $P_i : \R^{m_i} \rightarrow \R^{n_i}$ for layer $i$.
            \item Train \(S_i\) for \(t_i\) iterations to reduce the MSE loss between \(S_i(x)\) and \(P_i(T_i(x))\):
            $\mathcal{L}_i = \frac{1}{T} \sum_{t=1}^{T} \| S_i(x^{(t)}) - P_i(T_i(x^{(t)})) \|^2_2$
            where $T$ is the number of training samples.
        \end{enumerate}
    \item 
    Train the entire student network $S$ for $t_L$ iterations to reduce the KL-divergence loss between $S(x)$ and $T(x)$.
\end{enumerate}
\end{definition}



\section{Learning Sparse Parities via Curriculum Extraction}
\label{sec:sparse_parities}


To demonstrate the effectiveness of our curriculum extraction scheme, we study its performance in learning sparse parities. 
We compare our curriculum extraction scheme to one-shot distillation, where the student is trained directly on samples generated by the teacher. 
%In \Cref{subsec:prelims} we define the problem and our setup.
%In \Cref{subsec:proof_overview} we give a brief overview of the proof. 
%In \Cref{subsec:sparse_parity_experiments} we demonstrate our experimental results on transformer and MLP architectures. 
% we will briefly present our main theorem (a formal version of \Cref{thm:main_informal}) and outline the proof. 

% We also study this experimentally by training MLP and transformer models.

%\subsection{Theoretical Analysis}

\subsection{Preliminaries}
\label{subsec:prelims}

% We study the performance of our curriculum extraction scheme in the stylized context of learning the problem of sparse parities as defined in \Cref{prob:sparse_parities}. 
For our arguments in this section, we will assume WLOG that the support of the unknown parity is $S = [k]$. 
We will learn two-layer MLP networks of the form 
$f(\bx) := \ba \cdot \sigma(\bW \bx + \bb) = \sum_{i=1}^m a_i \sigma(\bw_i \cdot \bx + b_i)$. 
where $\bx \in \R^d; \bW \in \R^{d \times m}$; $\bb, \ba \in \R^m$, and $\sigma(t) := \max(0, t)$ is applied coordinate-wise when applied to a vector. 
We will denote the student network by $f_s$ and the teacher network by $f_t$ with hidden dimensions $m_s$ and $m_t$ respectively.
In general $m_s \leq m_t$. 
Let $\ell_f(\bx, y) := \max(0, 1-f(\bx)y)$ be the hinge loss. 
Our main task will be to find the best fitting two-layer MLP to an unknown sparse parity function. 

\begin{problem}[Learning Sparse Parities]
\label{prob:sparse_parities}
    Let \( S \subset [d] \) with \( |S| = k \) and \( k < d \) denote the support of our unknown sparse parity. 
    For \( \bx \in \{\pm 1\}^d \), we define $\chi_S(\bx) := \prod_{i \in S} x_i$ to be a \emph{sparse parity} supported on $S$.  
    Given a tolerance \(\epsilon \in \R\) and $n$ samples \(\{(\bx_i, \chi_S(\bx_i)) \mid \bx_i \sim_{u.a.r} \{\pm 1\}^d \text{ for } i \in [0, n]\}\) for an unknown support $S$, 
    the task of learning a sparse parity function using a two-layer MLP, is to find a two-layer MLP that achieves loss $\E_{(\bx, y)} [\ell_f(\bx,y)] \leq \epsilon$. 
\end{problem}


For our theoretical analysis, our training setup differs slightly from \Cref{def:scheme} when it comes to our losses -- we use a regularized version of the hinge loss to train the bottom layer of the teacher, the hinge loss to train the top layer of the teacher as well as the student, and a regularized version of a correlation-based distillation loss (defined below) to train the student's hidden layer.

\paragraph{Initialization}
Prior to training, we will initialize the network using the following symmetric initialization from \citet{barak2022hidden}.

\begin{definition}[Symmetric Initialization]
\label{def:sym_initialization}
Let $f(\bx) := \sum_{i=1}^m a_i \sigma(\bw_i \cdot \bx + b_i)$ be a two-layer MLP with input dimension $d$ and hidden dimension $m$. For each 
$1 \leq i \leq m/2,$ we initialize the parameters $\{\bw_i\}_{i=1}^m$, $\{b_i\}_{i=1}^m$ and $\{a_i\}_{i=1}^m$ as follows: $\bw_i \sim U(\{\pm 1\}^d),$
$b_i \sim U\left(\left\{-1 + \frac{1}{k}, \cdots, 1 - \frac{1}{k}\right\}\right), 
\quad a_i \sim U\left(\left\{\frac{\pm 1}{m}\right\}\right)$, $m/2 < i \leq m$ are set to $\bw_i = -\bw_{i -m/2}, \quad b_i = b_{i -m/2}, \quad a_i = -a_{i -m/2}$.
\end{definition}


\paragraph{Training Algorithms:}
We train the teacher network $f_t$ by minimizing the hinge loss in two stages. 
In the first stage of training, we freeze the top layer weights $(\ba)$ and train the network with a regularized version of $\ell_{f_t}(\bx, y)$, given by $\ell_{f_t}(\bx, y) - \lambda \|\bW\|^2$ updating only $\bW$.
In the second stage of training, we freeze the bottom layer weights and biases $\bW, \bb$ and only update $\ba$. 

For the student network $f_s$, we define a \emph{distillation loss} instead.
Let $f_t^{(1)} := \sigma(\bW \bx + \bb) : \R^d \rightarrow \R^{m_t}$ denote the output of the first layer of the teacher and suppose $A \in \R^{m_t \times m_s}$ is a random symmetric projection which mimics the initialization, i.e. for $i \leq m_t/2$, each \new{$A_{ij} \sim U(\{\pm 1/m_t\})$} and for $i > m_t/2$, 
$A_{ij} = -A_{(i-m/2)~j}$.
In the first stage (where we only update the bottom layer weights), the first layer of the student (i.e. $f_s^{(1)}(\bx) := \sigma(\bW_s \bx + \bb_s)$) is trained using the a similarly regularized version of the following distillation loss: 
$\ell_{DL}(\bx, f_s^{(1)}, Af_t^{(1)}) = \new{-f^{(1)}_s(\bx) \cdot (Af^{(1)}_t(\bx))}$, i.e. we use the loss $\ell_{DL}(\bx, f_s^{(1)}, Af_t^{(1)}) - \lambda \|\bW_s\|^2$ for a carefully chosen value of $\lambda$.
% \max(0, 1 - f^{(1)}_s(\bx) \cdot (Af^{(1)}_t(\bx))).

The second layer of the student ($\ba_s$) is then trained using the standard hinge loss.

\subsection{Theoretical Results}
\label{sec:main-thm}
We prove that, compared to one-shot distillation—where the student needs at least \(\Omega\left(d^{k-1}\right)\) samples to learn the unknown sparse parity—our curriculum extraction method reduces this requirement to \(\tilde{O}(2^{O(k)}\poly(k,d))\).
We state this formally below:
\begin{theorem}[Curriculum Extraction Requires Fewer Samples]
\label{thm:main}
    Let $m_s$ and $m_t$ denote the student and teacher hidden dimensions, with $m_t \geq \Omega(m_s^2 k^2)$ and $d \geq \Omega(m_s k^4)$,
    Suppose the teacher model 
    % (having a hidden dimension of size $m_t$)
    % \new{(of size $O(2^{O(k)}\poly(d, k))$)} 
    has been trained to learn a $d$-dimensional $k$-sparse parity with the 2-stage training algorithm in \Cref{alg:2_stage_training},
    % , which satisfies the conditions in \Cref{lem:effect_of_1_step_on_w} at the end of the first stage 
    % \new{for hidden layer size $m_t \leq d^{k-1}$} 
    and achieves a loss of $O(d^{-c})$ for some constant $c \geq 1$ at the end of the second stage. 
    Suppose further, that we train a student model $f_s$ of size $m_s = \tilde{\Theta}(2^k k)$ using the following two strategies:
\begin{enumerate}
    \item \textbf{Random-projection curriculum extraction:} 
    Train the first layer of the student with a random projection of the first layer of the teacher to the right output dimension, and then train the entire student network with the final teacher network.
    \item \textbf{One-shot Distillation:} Train with the teacher network throughout.
\end{enumerate}

Then,
\begin{enumerate}
    \item 
    \label{item:sufficient_our_distillation_scheme}
    Under our distillation scheme, the total sample complexity to reach a loss of $\epsilon$ with probability $99\%$ is 
    % $\Theta(2^{O(k)} \poly(d,k)\epsilon^{-2} \log(k/\delta\epsilon)).$
    $\Theta(2^{O(k)} \poly(d,k)\epsilon^{-2} \log(k/\epsilon)).$
    \item The necessary sample complexity under distillation is at least
    \label{item:necessary_one_shot_distill}
    $\Omega\left(d^{\min(2c, k-1)}\right)$.
    
\end{enumerate}
% Then, (1) Under our distillation scheme, the total sample complexity to reach a loss of $\epsilon$ with probability $1 - \delta$ is $\Theta(2^{O(k)} d^2 \epsilon^{-2} \log(k/\delta\epsilon)).$ (2) The necessary sample complexity under distillation is at least
    % $\Omega\left(d^{\min(2c, k-1)}\right)$.
\end{theorem}
 The key difference between the two is that, in one-shot distillation, the student must identify one of \(\Omega(d^k)\) possible parity functions from scratch. In contrast, our scheme splits the learning into two phases: identifying the support and learning the final function. Initially, the gradients of the distillation loss guide the student in detecting the support of the sparse parity via the bottom layer. With the support identified, the student only needs to select from \(O(2^k)\) possible parities.

\subsubsection{Proof Overview}
\label{subsec:proof_overview}

% In this section, we prove our main theorem which states that, compared to one-shot distillation—where the student requires at least $\Omega\left(d^{\min(2c, k-1)}\right)$ samples to learn the unknown sparse parity—our curriculum extraction method reduces the sample requirement to $\tilde O(2^{2k})$.

% To understand why this is the case, consider the difference in what the student must learn between the two situations. With one-shot distillation, the student has to learn one of $\Omega(d^k)$ possible parity functions that the teacher could be approximating and must identify the correct one from scratch.
% , greatly reducing the required sample size.
% \new{SK: Integrate this difference again into the rest, labels are broken now.}
% \new{SK: Fix algorithm enviornment in appendix.}
% \new{SK: Fix prose to connect with fact we don't have to main theorem.}

% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     \begin{minipage}[b]{0.5\linewidth}
%         \centering
%         \includegraphics[width=1\textwidth]{unpolished_figs/mlp_correlation.pdf}
%         % \caption{(a)}
%         \label{fig:mlp_correlation}
%     \end{minipage}
%     % \begin{minipage}[b]{0.8\linewidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
%     % \caption{MLP Student Accuracy}
%     % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     % \hfill
%     \caption{%
%     \textbf{In-support and out-of-support correlations.} 
%     % \new{in progress... }
%      A two-layer MLP trained on 100-dimensional 6-sparse parity data exhibits distinct in-support (red) and out-of-support (blue) correlations of $(Af_t^{(1)})(\bx)$ with $x_j$ for the random projection $A \in \R^{1 \times m_t}$. When $j$ is in the support, the correlations show significantly larger standard deviations compared to when $j$ is outside the support. 
%     }
%     \label{fig:correlation_plot}
% \end{figure}


% \subsubsection{Proof Overview}
% \new{SK: Back here.}

We begin by assuming, without loss of generality, that the support of the unknown parity is $S=[k]$. 
Our goal is to prove two main results: a lower bound for one-shot distillation and an upper bound on the sample complexity of our curriculum extraction scheme. 
The lower bound follows directly from \citet{panigrahi2024progressive} (Theorem B.1); here we focus on a high level sketch of the upper bound.

% Without loss of generality, suppose that the support of the unknown parity $S = [k]$. 
% The lower bound on the sample complexity for one-shot distillation (\Cref{item:necessary_one_shot_distill} in \Cref{thm:main}) 
% follows from the exact same item in the analogous result in \citet{panigrahi2024progressive} (Theorem B.1). 
% The rest of this section will focus on a high-level sketch of a sample complexity upper bound of $\tilde O(2^{O(k)} \poly(k,d))$ for our curriculum extraction scheme (i.e. \Cref{item:sufficient_our_distillation_scheme} in \Cref{thm:main}). 

To achieve this, our approach explicitly separates two tasks: first, \emph{support recovery} (identifying the relevant coordinates for the 
$k$-sparse parity), and second, \emph{loss minimization} (optimizing the network to approximate the parity function). This separation is central to reducing the sample complexity. 

Our key insight is to exploit a property of the teacher's first-layer weights. When the teacher is trained using the two-stage process, the first-layer weights have significantly larger magnitudes on the true support than on the out-of-support coordinates (see \Cref{lem:effect_of_1_step_on_w}). This gap is crucial for ensuring that the second stage of training can find a network with low loss.
% Our key insight is to exploit a property of the teacher's first-layer weights. When the teacher is trained to achieve a loss using the two-stage training process, its first-layer weights exhibit significantly larger magnitudes on the true support compared to the out-of-support coordinates (see \Cref{lem:effect_of_1_step_on_w}). This gap is critical for the second stage of training to be able to find a network achieving a small loss. 
In particular, Theorem 4 from \citet{barak2022hidden} (restated in \Cref{lem:second_stage_conclusion}) shows that the \(k\)-sparse parity can be accurately approximated by training only the top layer of the student, provided that the hidden layer is large enough (at least \(\tilde{\Omega}(2^k k)\)) and when there is a clear gap between the in-support and out-of-support coordinates of the weights at the end of the first stage of training.

In our approach, we transfer the gap from the teacher to the student's first-layer weights using the gradients of the distillation loss during the first training step. This transfer enables support recovery using far fewer samples than would be required if we trained the entire network from scratch. Once the support is recovered, the second stage of training, where we update only the top layer weights, proceeds exactly as in \cite{panigrahi2024progressive, barak2022hidden}.

Because the student's first layer \(f_s^{(1)}\) can only learn about the support through the gradients of the distillation loss, we choose an appropriate regularization parameter \(\lambda\) so that the student's weights become proportional to these gradients after the first update. This means that it is sufficient to demonstrate a clear gap between the magnitudes of the in-support and out-of-support coordinates of the gradient at initialization. In fact, \Cref{lem:teach_gap_implies_student_gap} shows that the gradient of the distillation loss with respect to \(\bw_i\) is proportional to
$\E_{\bx}\Bigl[(Af_t^{(1)}(\bx))_i \, \bx + (Af_t^{(1)}(\bx))_i \, \maj(\bw_i \odot \bx)\, \bx\Bigr].$
Thus, if we can show that the magnitude of the $j$-th coordinate for $j \in S$ (in-support) is significantly larger than for $j \notin S$ (out-of-support) the student can effectively recover the support from the gradient information.
For the remainder of this discussion, we focus on showing this gap for the first term, since it will turn out that the second term is dominated by this first term.

The \(j\)-th coordinate of the first term is given by $\E_{\bx}\Bigl[(Af_t^{(1)}(\bx))_i\, x_j\Bigr].$
It turns out that due to the symmetric initialization, the weights after the first stage of training inherit this symmetry (see, \Cref{lem:effect_of_1_step_on_w}).
As a result, we can rewrite the first term as a sum of scaled Rademacher random variables \(\{A_{i\ell}\}_{\ell=1}^{m_t/2}\), 
$\E_{\bx}\Bigl[(Af_t^{(1)}(\bx))_i\, x_j\Bigr] 
% = \sum_{\ell=1}^{m_t} A_{i\ell}\,\E_{\bx}\Bigl[\sigma(\bx\cdot \bw_\ell + b_\ell)x_j\Bigr]
= \sum_{\ell=1}^{m_t/2} A_{i\ell}~\E_{\bx}\Bigl[\left( \sigma(\bx\cdot \bw_\ell + b_\ell) - \sigma(-\bx\cdot \bw_\ell + b_\ell) \right)~x_j\Bigr]$.
This representation is particularly useful, because, by the central limit theorem, the sum of scaled Rademacher random variables behaves like a mean-zero Gaussian with variance $\sigma_j^2 := \sum_{\ell=1}^{m_t/2} s_{\ell j}^2/m_t^2,$
where $s_{\ell j}$ are scaling factors defined as, $s_{\ell j} := \E_{\bx}\Bigl[\left( \sigma(\bx\cdot \bw_\ell + b_\ell) - \sigma(-\bx\cdot \bw_\ell + b_\ell) \right)~x_j\Bigr]$.
\Cref{lem:bounds_on_coeffs} then guarentees that the scaling factors are significantly larger when \(j\) is in the true support \(S\) than when \(j\) is not. 
This, in turn, 
% \Cref{lem:bounds_on_coeffs} 
% (from \cite{panigrahi2024progressive}) 
implies that the standard deviations of the in-support $j$ are much larger than those for the out-of-support $j$, more precisely, $\sigma_j > \frac{1}{k\sqrt{m_t}}$ for $j$ in the support, and $\sigma_j < \frac{1}{kd\sqrt{m_t}}$ for $j$ out of the support (see \Cref{fig:correlation_plot} for the corresponding distributions in our trained network). 


% However, we must consider the full sum of these scaled Rademacher random variables. By the central limit theorem, this sum is well-approximated by a mean-zero Gaussian with variance $\sigma_j^2 := \sum_{\ell=1}^{m_t/2} s_{\ell j}^2/m_t^2,$
% as also illustrated in \Cref{fig:correlation_plot}. 

Next, by applying anticoncentration and concentration inequalities for sums of Rademacher random variables
- which behave similar to those of a Gaussian - to the sum
$\sum_{\ell=1}^{m_t/2} A_{i\ell} s_{\ell j}$
we show that, with high probability over the randomness of the projection $A$, this variance gap carries over to a proportional gap in the coordinates of $\E_{\bx}\Bigl[(Af_t^{(1)}(\bx))_i\,\bx\Bigr]$ 
% for a fixed draw of \(A\)
. This result is summarized informally below; the formal statement of which is provided in \Cref{lem:degree_1_gap}.


% XXX THIS MIGHT BE IMPORTANT TO BRING BACK. 
%
% For the sake of illustration, consider the unknown sparse parity $\chi_{[k]}(\mathbf{x}) := \prod_{i=1}^k x_i : \{\pm1\}^d \to \{\pm1\}$. Our goal is to learn this function using a two-layer MLP. 
% First, note that the parity function \(\chi_{[k]}(\mathbf{x})\) can be \emph{represented} by a reasonably sized two-layer MLP. Since \(\chi_{[k]}(\mathbf{x})\) depends only on the sum \(\sum_{i=1}^k x_i\) due to its symmetry in \(x_1, \dots, x_k\), it can be rewritten as \(\chi_{[k]}(\mathbf{x}) = g\left(\sum_{i=1}^k x_i\right)\) for a univariate function \(g(t)\) mapping integers between \(-k\) and \(k\) to \(\{\pm 1\}\). A two-layer MLP with \(O(k)\) ReLU activations can approximate this function by constructing a piecewise linear function over the \(2k+1\) possible values.

% If the ambient dimension is $d \gg k$, then this neural network may be realized by simply setting the out-of-support coordinates of the weight vectors to be $0$. 
% Hence, if you know the parity apriori, it is easy to construct the two-layer MLP that represents it.

% In fact, it is possible to approximate the unknown sparse parity when much less is known --- 
% Theorem 4 from \citet{barak2022hidden} shows that the \(k\)-sparse parity can be well-approximated by training only the top layer, given a hidden dimension of size \(\tilde{\Omega}(2^kk)\) and random weights, provided there is a gap between in-support and out-of-support variables of the bottom layer weights. We restate the version of this theorem from \citet{panigrahi2024efficient} in \Cref{lem:second_stage_conclusion}.
% }


\begin{lemma}[Correlation Gap (Informal)]
\label{lem:corr_gap_informal}
% As long as 
% $m_t ~\new{ = 2^{O(k)}\poly(d,k)/\delta^2} \geq (m_s^2 ~k^4 \log(d)^2 / \delta^2)$, 
Let $d \geq \Omega(m_s k^4)$ and $m_t \geq \Omega(m_s^2 k^2)$. 
Then, with probability 
% $1-\delta$
$99\%$ over the randomness of initialization, \emph{every} coordinate $i \in [m_s]$ of the projected teacher network satisfies $\left|\E_\bx[(Af_t)_i (\bx) x_j]\right| > \Omega((k^2 m_s \sqrt{m_t})^{-1})$ for all $j$ in the support of the unknown sparse parity, and $\left|\E_\bx[(Af_t)_i (\bx) x_j]\right| \leq O((k^3 m_s \sqrt{m_t})^{-1})$ for $j$ that are out-of-support.
% Let $f(\bx) := \sum_{i=1}^{m_t} a_i \sigma(\bw_i \cdot \bx+b_i)$ and $f^r(\bx) = \sum_{i=1}^{m_t} a^r_i \sigma(\bw_i \cdot \bx+b_i)$,
% where $a_i^r$ and $a_i^{(0)}$ are independently drawn u.a.r. from $U(\{\pm 1/m\})$ for $i \in [m_t/2]$ and $a^r_{i+m_t/2} = -a^r_i$, 
% and $a_i^{(0)}$ and $\bW^{(0)}$ are initialized according to the initialization scheme in \Cref{subsec:prelims}.
% Let $m_t \geq \Omega(k^4 \log(d)^2/\delta^2)$, then
% \[ \min_{j \in [k]} \left|\E_\bx[f^r(\bx) x_j]\right| > \frac{1}{m_tk} \text{ and } \max_{j > k} \left|\E_\bx[f^r(\bx) x_j]\right| < \frac{1}{m_tkd}\]
\end{lemma}

Next, we focus on the gradient gap that drives the support recovery. Our aim is to establish a gap between the in-support and out-of-support coordinates of the gradient, which is proportional to $\E_{\bx}[(Af_t^{(1)}(\bx))_i \, \bx + (Af_t^{(1)}(\bx))_i \, \maj(\bw_i \odot \bx)\, \bx]$. 
Above, we outlined the argument to show a gap for the first term. 
\Cref{lem:expansion_of_f_r} further demonstrates that the second term is dominated by the first, 
and so this gap transfers to the gradient.

% Our discussion above establishes the gradient gap in expectation, 
% We now address its empirical counterpart.
Now, we must verify that this gap persists when using empirical estimates. To do so, it is sufficient to ensure that the scaling factors of the variables $\{ A_{i\ell} \}_{\ell=1}^{m_t/2}$, are close to the true expectations.
If this closeness holds, the empirical standard deviations will inherit the gap observed by the $\sigma_j$, and the concentration and anticoncentration properties will continue to apply -- thus preserving the conclusion of \Cref{lem:corr_gap_informal}.
% This ensures that the standard deviations of the empirical estimates
% , $\hat \sigma_j := \sum_{\ell=1}^{m_t} \widehat \E_{\bx}\Bigl[\sigma(\bx\cdot \bw_\ell + b_\ell)x_j\Bigr]^2$, 
% continue to see the gap that was witnessed by $\sigma_j$, allowing the anticoncentration and concentration properties of $\E_\bx [(Af_t^{(1)}(\bx))\bx]$ over the randomness of $A$ to continue to hold, which in turn maintains the conclusion of \Cref{lem:corr_gap_informal}.
% to continue to hold, the empirical estimate are similar to those of the true expectation.

In \Cref{lem:emp_grad_gap}, we use Hoeffding's inequality (\Cref{lem:hoeffding}) to show that the empirical scaling factors converge to their true values with only $O((kd)^2 \log(m_td))$ samples. Once the gradients are updated using these empirical estimates, the student's weights exhibit a gap -- after rescaling by $m_s \sqrt{m_t}$ this gap is $\Omega(1/k^2)$.
This result allows us to invoke the analysis from \cite{barak2022hidden, panigrahi2024progressive} for the second stage, which requires an additional $\tilde O(2^{O(k)}\poly(d)/\eps^2)$ samples to achieve a loss of $\eps$. Thus, we learn the parity with a significantly smaller overall sample complexity compared to one-shot distillation.

At this point, we note an important difference between our proof and the one for progressive distillation in \citet{panigrahi2024progressive}. In their work, the weights after the first stage of training adjust to the initialized top layer. This dependence allows them to more easily demonstrate a gap in the gradients, without having to deal with the randomness of a projection. In fact, we also observe the effect of being able to tune to the current top layer in \Cref{fig:student_accuracies} (a), where we see that progressive distillation is able to make some progress even during the stage where we only tune the bottom layer weights. 
In our setting, in the first phase of training, we train the bottom layer of the student independently of the top layer, requiring us to rely on a different argument.

% Now, the only way for the first layer of the student to get information about the support from the hidden layer of the teacher is through the gradients of the distillation loss. 
% By a careful choice of the regularization parameter (as done in \citep{barak2022hidden,panigrahi2024progressive}), the weights after the first step actually turn out to be proportional to the gradients itself. 
% We show that these gradients essentially end up depending on the Fourier coefficients of the output of the hidden student dimension -- more precisely \Cref{lem:teach_gap_implies_student_gap} shows that the gradient of the distillation loss with respect to $w_{ij}$ is proportional to the sum of the $j$-th degree-1 Fourier coefficients of the $i$-th coordinate of the random projection of the hidden layer $(Af_t^{(1)})_i$, and $\maj(\bw_i \odot \bx) (Af_t^{(1)})_i$. Since the in-support coordinates of the teacher weights are larger than the in-support coordinates, It so happens that if all the layer-1 teacher weights have a gap between the in-support coordinates and out-of-support coordinates, 
% then these Fourier coefficients also have a gap -- In \Cref{lem:degree_1_gap} we show that randomly projecting the teacher's first-layer weights to the student's hidden dimension preserves this gap with high probability, 
% creating a smaller but proportional gap in the absolute values of the teacher network's degree-1 Fourier coefficients (see \Cref{fig:correlation_plot} for the distributions of the in-support and out-of-support variables of our trained network).
% The gap in the distillation loss gradient is a constant multiple of this gap (\Cref{lem:teach_gap_implies_student_gap}). 
% The final sample complexity needed to learn this is a function of is gap.
% Unfortunately, in our case since such a property does not hold (i.e. the random projection is independent of the teacher weights) we have to use a different strategy.
% We show that, under the randomness of the projection, each coordinate of the projected teacher hidden dimension can be represented as a sum of Rademacher random variables, with variances significantly higher for in-support coordinates compared to out-of-support coordinates. 
% Using anticoncentration and concentration inequalities for sums of random variables, we establish that, with reasonable probability over the randomness of the top layer weights, this variance gap translates into an actual value gap in the degree-1 Fourier coefficients. 
% At this point we note an important difference between our proof and the one in \citep{panigrahi2024progressive}. 
% In their paper, the weights after the first stage of training have signs that match the top-layer coefficients, this allows them to easily show that the population gap is large, since there is no randomness in the final student weights. 
% Unfortunately, in our case since such a property does not hold (i.e. the random projection is independent of the teacher weights) we have to use a different strategy.
% We show that, under the randomness of the projection, each coordinate of the projected teacher hidden dimension can be represented as a sum of Rademacher random variables, with variances significantly higher for in-support coordinates compared to out-of-support coordinates \new{(see \Cref{fig:correlation_plot} for the distributions of the in-support and out-of-support variables of our trained network)}. Using anticoncentration and concentration inequalities for sums of random variables, we establish that, with reasonable probability over the randomness of the top layer weights, this variance gap translates into an actual value gap in the degree-1 Fourier coefficients. 
% Once we establish such a gap, it is easy to show that the gradients inherit this gap (which follows from \Cref{lem:expansion_of_f_r}). 
% Except for the calculations for the correlations with degree-1 coefficients, the rest of the proof follows similar to that in \citep{panigrahi2024progressive}. 
% The proof of \Cref{thm:main} follows from demonstrating a Fourier gap in the sense of \Cref{prop:fourier_gap_implies_recovery}.
% For the sake of illustration, suppose the unknown sparse parity is $\chi_{[1,2,3]}(\bx) := x_1x_2x_3 : \{\pm 1\}^d \rightarrow \{\pm 1\}$. 
% Our aim is to learn this using a depth-2 ReLU network. \newline
% First note that since $\chi_{[1,2,3]}(\bx)$ is a symmetric function in $\bx$, it only depends on $x_1+x_2+x_3$, but not on the specific permutation \new{SK: does this need a citation?}. 
% This fact allows us to think of $\chi_{[1,2,3]}(\bx)$ instead as a univariate function $g(t):\R \rightarrow \{\pm 1\}$, where
% $\chi_{[1,2,3]}(\bx) = g(x_1+x_2+x_3)$. 
% it is well-known that we can approximate any depth-two neural network taking $6$ values using $12$ neurons (just use the ReLU network to match a piecewise linear function going through the specific output values for different input values). 
% Hence, if the support is known, it is quite easy to find the right set of neurons to do the job. 
% Theorem 4 from \citep{barak2022hidden} (which we restate in \Cref{lem:second_stage_conclusion}) shows that the second stage of training (for the teacher and the student) works as long as there are at least $\Omega(2^{k}k\log(k))$ hidden layer neurons and the in-support and out-of-support coordinates of the weights of the first layer have a gap. 
\subsection{Experiments} 
\label{subsec:sparse_parity_experiments}
% \new{SK: Here now, will continue in some time to have fresh eyes.}
We investigate curriculum extraction for the problem of learning sparse parities for a Multi-Layer Perceptron (MLP) and Transformer architectures, which we describe below:
% \new{TODO: description of compute we run the experiment on}

\paragraph{Student and Teacher Architectures}
For the \emph{Multi-Layer Perceptron,} both the student and teacher are two-layer MLPs with the teacher network having a hidden dimension of $5 \times 10^4$ and the student having hidden dimension $100$.  For the \emph{transformer architecture}, the transformer configuration has matching embedding dimensions ($256$ dimensions for both teacher and student); however, the teacher has 32 attention heads and the student has only 4. \new{Both student as well as teacher architectures use two decoder blocks followed by a linear projection layer.}
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{figures/mlp_correlation.pdf}
%         \caption{MLP hidden state alignment}
%         \label{fig:mlp_corr}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{figures/transformer_correlation.pdf}
%         \caption{Attention pattern similarity}
%         \label{fig:trans_corr}
%     \end{subfigure}
%     \caption{Representation similarity analysis showing (a) Pearson correlation $r=0.92$ between teacher (50k-dim) and student (100-dim) MLP hidden states, and (b) cosine similarity 0.87 in attention patterns between teacher (32-head) and student (4-head) transformers. Gray dashed lines indicate layer correspondences established through our curriculum.}
%     \label{fig:correlation_plots}
% \end{figure}
\paragraph{Training and Evaluation}
Our distillation loss is the Mean Squared Error (MSE) and the final checkpoint training is done using the Cross-Entropy loss. 
We measure performance of our model by looking at the accuracy. 
% \new{SK: this needs a more detailed description... specifically how we train the transformer and the MLP..  }
\subsubsection{Discussion}
\paragraph{Multi-Layer Perceptron:}
In \Cref{fig:student_accuracies} (a), we compare the performance of MLPs trained using one-shot distillation, layer-wise curriculum extraction, and the progressive distillation approach from \citet{panigrahi2024progressive}. In both curriculum extraction and progressive distillation, we switch to the final checkpoint at iteration \( 5 \times 10^5 \).

We observe that after \(10^6\) iterations, both methods perform comparably, with progressive distillation achieving slightly higher accuracy. Notably, progressive distillation shows early improvement before the \(5 \times 10^5\) iteration mark, likely due to the MLP's bottom layer quickly tuning to the top layer. In the second phase of training, the top layer benefits from a well-optimized starting point. 
% Towards the end, both perform comparably.
% We observe that both perform comparably after $10^6$ iterations, with progressive distillation achieving very slightly higher accuracy. 
% We also see that progressive distillation begins improving before the \( 5 \times 10^5 \) iteration mark. 
% This early improvement is likely due to the fact that in progressive distillation, the bottom layer weights of the MLP tune themselves to the top layer, and the overall network begins to see improved performance right away. 
% Once the top layer is activated, it benefits from a well-optimized starting point tailored to itself. 
With curriculum extraction on the other hand, the bottom layer starts randomly initialized and uncorrelated with the top layer, limiting early gains. However, once we begin training the top layer, performance improves rapidly, matching progressive distillation. In contrast, one-shot distillation shows no significant improvement, even after \(2 \times 10^6\) iterations.
In fact, we observe in \Cref{fig:mlp_proj_vs_layer_correlation} that 
% even though the final network for curriculum extraction appears to have low loss in the first \( 5 \times 10^5 \) iterations, 
% it appears that 
our curriculum extraction method leads to the more information about the support being transferred to the underlying network than progressive distillation.


% In contrast, with curriculum extraction, the bottom layer cannot directly leverage any pre-trained information from the top layer, since it is randomly initialized and remains uncorrelated with the bottom layer during the first phase of training. 
% However, once the top layer begins training at iteration \( 5 \times 10^5 \), the performance of the curriculum extraction method improves rapidly, quickly reaching accuracy levels comparable to those of progressive distillation. 
% On the other hand, the one-shot distillation method shows no significant gains, even at \( 2 \times 10^6 \) iterations.

    
\paragraph{Transformer:}
In \Cref{fig:student_accuracies} (b), we compare the performance of the transformer model trained using one-shot distillation and our curriculum extraction scheme, with a checkpoint at $10^5$ iterations. We see that this leads to significantly improved student performance over the one-shot distillation case. 
% \new{XXX Anything else to say here?}

% \new{
% \begin{enumerate}
%     \item Figure 3 is plotting this. 100, 6 exactly same. Take the bottom layer and project it onto one dimension look at correlation of.. fourier coeffiients. 
%     \item Figure 2 -- 3 plots next to each other figure.  
%     \item Progressive thing seems like it gets higher accuracy but this is because top layer is being trained simultaneously with the bottom layer. 
%     \item 50k mark we switch over to final checkpoint. 
%     \item curriculum extractin doesn't give you accuracy increase until you switch to the final layer, top layer is random u don't expect any increase.. can write formally. top layer is random combination of bottom layer. 
%     \item what we really care about how much bottom layer has learnt and can plot correlation etc -- point to appendix with the correct plot
% \end{enumerate}
% }


% The curriculum's phased approach proves essential, as demonstrated in Figure~\ref{fig:progressive_vs_layerwise}. For MLPs, progressive training achieves $92\%$ final accuracy compared to 68\% for direct layerwise optimization—a gap attributable to the student's need to gradually assimilate information from the teacher's massive 50k hidden layer. Transformers reveal complementary dynamics: early training phases are dominated by MSE loss (4.2$\times$ reduction in Phase 1) as the 4 student heads learn to mimic critical subsets of the teacher's 32-head attention patterns, before cross-entropy optimization finalizes the random projection layer's outputs.

% Implementation critically depends on three design choices: random projection initialization for the student's embedding layer, LayerNorm stabilization before MSE computation to handle dimension mismatches, and head importance-based pruning (Appendix~\ref{app:head_prune}) that identifies which of the teacher's 32 heads to prioritize during each curriculum phase. These mechanisms enable effective knowledge transfer despite the student's severe capacity constraints—the MLP student operates with $0.2\%$ of the teacher's hidden dimension, while the transformer must collapse 32 attention heads into 4 without losing critical pairwise token interactions.



\section{BERT Language Modeling}
\label{sec:bert}
\begin{figure*}[t]
    \centering
    %--------------------
    % First subfigure
    %--------------------
    \begin{minipage}[t]{0.31\linewidth}
        \centering
        \hspace*{-2mm}
        \includegraphics[width=1.1\textwidth]{unpolished_figs/bert_pcfg_flops_vs_acc.pdf}
        \vspace{0.3em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(a)} % Manually add caption
        \label{fig:bert_pcfg_flops_vs_acc}
    \end{minipage}
        \hfill
        \begin{minipage}[t]{0.31\linewidth}
    \centering
    \hspace*{-2mm}
    \includegraphics[width=1.1\textwidth]{unpolished_figs/bert_pcfg_layerwise_vs_oneshot_acc.pdf}
        \vspace{0.3em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(b)} % Manually add caption
    \label{fig:many_vs_one_bert_pcfg}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.31\linewidth}
    \centering
    \hspace*{-3mm}
    \includegraphics[width=1.1\textwidth]{unpolished_figs/many_vs_one_bert_pcfg.pdf}
        \vspace{0.3em} % Adjust spacing as needed
        \centering\scriptsize\textbf{(c)} % Manually add caption
    \label{fig:bert_pcfg_layerwise_vs_oneshot_acc}
    \end{minipage}

    \caption{%
    \textbf{PCFG Experiments on BERT.}
    The dashed vertical lines indicate iterations where the layer being distilled from is changed.
    % , in the case of curriculum extraction.
    (a) Soon after the final checkpoint, curriculum extraction achieves a larger accuracy in the same number of FLOPs, when compared to one-shot distillation.
    (b) We compare curriculum extraction to one-shot distillation across three models trained with two, three, and four-stage curricula at 4000, 6000, and 8000 iterations, respectively. Curriculum extraction consistently outperforms one-shot distillation at all scales. 
    (c) We compare curriculum extraction performance by varying the number of layers. With a fixed budget of 6000 iterations (2700 for extraction, 3300 for full network training), extracting from three layers outperforms one-shot distillation, and using a single layer.
    % We compare performance of curriculum extraction to one-shot-distillation for three models. The first one trained to 4000 iterations using a two-stage curriculum, the second one trained to 6000 iterations using a three-stage curriculum and the third model trained to 8000 iterations using a four-stage curriculum. At all these scales, we see that curriculum extraction outperforms one-shot distillation. 
}
    \label{fig:pcfg_bert}
\end{figure*}
We use BERT models trained for masked prediction, a task that involves predicting the tokens hidden (masked) in an input sequence. Similar to \citet{panigrahi2024progressive} we study this task for learning
probabilistic context-free grammars (PCFGs) and natural language modeling on the Wikipedia dataset. We define the masked token prediction task below.
% \new{TODO: description of compute we run the experiment on}
% ---well-known for effective feature learning in natural language \citep{hewitt2019,tenney2019,li2022}. 

\begin{problem}[Masked Token Prediction]
    Let $v$ be a vocabulary (including the token \([mask]\)), and let $x$ be a sequence of length $h$. We randomly choose a fraction $(30\%)$ of the positions $M\subseteq [h]$ to mask, with each position included independently with probability $p$. We create a masked input $x \setminus M$ by replacing tokens in $M$ with \([mask]\), a random token, or leaving them unchanged with respective probabilities $80\%,\,10\%,\,10\%$.
The model is then trained via a cross-entropy objective to predict the original tokens at those masked positions.
\end{problem}
For sequence-to-sequence modelling our teacher and student networks map from sequences to real vectors $f_t, f_s \colon v^h \;\to\; \mathbb{R}^{h \times C}$. The teacher’s output distribution at position $i$ is given by $p_T^{(i)}(\bx; \tau) \;=\; \mathrm{softmax}\bigl([f_t(\bx)]_i \,/\, \tau\bigr),$ and $p_S^{(i)}$ is defined analogously for the student.
% \new{Typically, we omit $\tau$ when $\tau = 1$.}
% \paragraph{Choice of Temperature} 
We set the temperature $\tau$ to $10^{-4}$ for experiments on sparse parity and PCFG, and to $10^{-20}$ for Wikipedia.
% for the Wikipedia experiments.

\paragraph{Training and Evaluation}
For the masked prediction task, we use $ \ell(\bx; f_S) = \mathbb{E}_{M} \Bigl[\frac{1}{|M|} \sum_{i \in M} \mathrm{KL}\bigl(e_{x_i} \,\|\, p_S^{(i)}(\bx \setminus M; \tau)\bigr)\Bigr],$ where $e_{y}$ is a one-hot vector with a 1 at index $y$ for the final layer training; and the MSE for the indetermediate layers as our distillation loss. Our final performance is measured using the top-1 accuracy on the masked tokens.

\paragraph{Student and Teacher Architectures}
For the \emph{PCFG tasks}, the teacher model uses a BERT-style architecture 
% designed for PCFG (Probabilistic Context-Free Grammar) tasks, 
with a 256-dimensional embedding, 32 attention heads, and 4 transformer blocks, trained with a batch size of 512. The student model retains the teacher’s 4-block architecture and 512 batch size but reduces the embedding dimension to 64 and the number of attention heads to 8.\\
For \emph{Wikipedia} language modeling, the teacher model follows a standard BERT-large configuration, with 768-dimensional embeddings, 12 attention heads, and 12 transformer blocks, trained with a batch size of 256. The student model preserves the teacher’s 12-block depth and 256 batch size but reduces the embedding dimension to 256  and the number of attention heads to 4.

\paragraph{Probabilistic Context-Free Grammar}
% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     \begin{minipage}[b]{0.8\linewidth}
%         \centering
%         \includegraphics[width=1\textwidth]{unpolished_figs/bert_pcfg_layerwise_vs_oneshot_acc.pdf}
%         \caption{BERT PCFG Accuracy}
%         \label{fig:bert_accuracy_pcfg}
%     \end{minipage}
%     % \begin{minipage}[b]{0.8\linewidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
%     % \caption{MLP Student Accuracy}
%     % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     \hfill
%      \caption{Layer-wise curriculum schedule showing progressive layer activation.}
%     \label{fig:bert_pcfg}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     \begin{minipage}[b]{0.8\linewidth}
%         \centering
%         \includegraphics[width=1\textwidth]{unpolished_figs/many_vs_one_bert_pcfg.pdf}
%         \caption{Comparing Curriculum extraction with using just the top layer's hidden representation to distill}
%         \label{fig:bert_accuracy_pcfg}
%     \end{minipage}
%     % \begin{minipage}[b]{0.8\linewidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
%     % \caption{MLP Student Accuracy}
%     % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     \hfill
%      \caption{Layer-wise curriculum schedule showing progressive layer activation.}
%     \label{fig:bert_pcfg}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{unpolished_figs/bert_pcfg_flops_vs_acc.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}
% \new{XXX -- PCFG formal sed to appendix, make informal here. }
A Probabilistic Context-Free Grammar (PCFG) generates sentences using a hierarchical tree structure, defined by non-terminal symbols, rules, a probability distribution over the rules, and a vocabulary of terminal symbols. PCFGs have been used as mechanistic proxies for language data \citep{panigrahi2024progressive, allen2023physics, zhao2023transformers}. We focus on masked token prediction for synthetic data from the cfg3b PCFG \citep{allen2023physics} (defined in \Cref{app:pcfg}). Our layer-wise curriculum schedule outperforms one-shot distillation. To confirm this improvement is due to the curriculum and not increased training bandwidth, we compare models trained with different curricula but the same time steps.

% A Probabilistic Context-Free Grammar (PCFG) generates sentences by following a hierarchical tree structure. 
% Specifically, a PCFG is defined by four components: a set of non-terminal symbols, a set of rules that operate on these non-terminals, a probability distribution over these rules, and a vocabulary of terminal symbols (words). 
% PCFGs have been used in \citep{panigrahi2024progressive, allen2023physics,zhao2023transformers} as mechanistic proxies for language data. 
% We study the task of masked token prediction for synthetic data generated by a specific PCFG from \citep{allen2023physics} --- cfg3b (more formally defined in \Cref{app:pcfg}).
% We observe that our layer-wise curriculum schedule outperforms one-shot distillation. 
% To ensure that it is indeed the curriculum and not increased bandwidth during training that leads to this improvement, we compare models that have been trained with different curricula but for the same number of time steps. 

% use these experiments to demonstrate that the reason for improved performance is the curriculum and not, for instance, 
% increased bandwidth during training. 
% \new{SK: need to describe what this is in words, and then smoothly transition.}
% Specifically, we study the often-used cfg3b grammar, defined in \Cref{app:pcfg}.

% \newpage

\subsection{Discussion}
\paragraph{PCFG Experiments:}

In \Cref{fig:pcfg_bert} (a), curriculum extraction shows FLOPS savings compared to one-shot distillation, outperforming it after \(\approx 0.8 \times 10^{13}\) FLOPS. Additionally, its accuracy improves at every checkpoint.

To establish that the reason for our improved performance is our scheme, 
In \Cref{fig:pcfg_bert} (b), we implement two distinct curriculum strategies for BERT distillation to train the student network while maintaining equivalent \emph{bandwidth} across our experiments.
We compare single-layer and multi-layer extraction, both with 6000 training steps and 2700 dedicated to curriculum extraction. The single-layer model uses one checkpoint at the end, while the three-layer model has checkpoints at 400, 1200, and 2700 steps. Extracting from three layers improves performance, while single-layer extraction appears to perform worse than one-shot distillation, possibly due to overfitting between the student's bottom layer and the teacher's upper layers.
% we compare single-layer extraction with multi-layer extraction -- in both settings we maintain a total budget of 6000 training steps, where the first 2700 are spent on curriculum extraction -- with only one checkpoint at the end for the single-layer extraction model, and with three checkpoints at iterations 400, 1200 and 2700 respectively for the three-layer extraction model. We see that extracting from three layers improves performance over extracting from a single layer. 
% In our figure, it appears to be the case that single layer extraction actually performs worse than one-shot distillation. \new{We suspect that this is because the bottom layer of the student in this case has somehow over-fit to the specific upper layers of the teacher.}

In \Cref{fig:pcfg_bert} (c) we see similar performance gains to those in \Cref{fig:pcfg_bert} (b) for higher bandwidth experiments -- for two, three and four-stage curricula. 
The two-stage curriculum skips the linear projection and first transformer layer for iterations 1 through 500, skips just the top linear layer for iterations \new{501 to 1500, and finally trains the entire network for iterations 1501 through 4000}.  
\new{The three-stage curriculum skips two encoder blocks for iterations 1 through 400, skips one encoder block for iterations 401 through 1200, and skips the final projection layer for iterations 1201 through 2700, finally training the entire network for iterations 2701 to 6000.}
The four-stage curriculum skips four encoder blocks for iterations 1 through 200, then three blocks for iterations 201 through 700, then two blocks for iterations 701 through 1500, one block for iteration 1501 through 3000 and finally just the final linear layer until iteration 8000.
% \begin{enumerate}
%     \item \emph{Single-Layer Extraction:}
    
%     % For 500 iterations we exclude the final layer and first transformer block
%     % For 1000 iterations we exclude only the final layer. 
%     % For the final 2500 iterations we train the entire network. 
%     % Finally, for the final 2500 iterations we train the entire network. 
%     \item \emph{Multi-Layer Extraction:}
    
%     % For 1500 iterations, we train the student network upto the penultimate layer (excluding the final layer),
%     % and for the final 2500 iterations we train the entire network. 
% \end{enumerate}
\paragraph{Wikipedia}
    In \Cref{fig:student_accuracies} (c) we see that our extraction scheme also works extremely well on real-world data.
    We train our BERT model for 500 iterations while skipping 4 encoder blocks, a further 1000 iterations while skipping 3 encoder blocks, a further 2000 iterations skipping one encoder block, 4000 iterations skipping the final projection layer and finally the full network for 16500 iterations.



% Note that here, we do not compare with one-shot distillation, but with two schemes having the same bandwidth, this shows us that the curriculum is what is contributing to our performance gains, and not just the (potentially) increased bandwidth. 

% For our 4K iteration baseline:
% \begin{itemize}
%     \item Phase 1 (500 iter): Skip final transformer layer
%     \item Phase 2 (1000 iter): Activate final layer
%     \item Phase 3 (2500 iter): Full network
% \end{itemize}

% This contrasts with na\"ive approaches that use:
% \begin{itemize}
%     \item 2700 iterations with random layer dropout
%     \item 3300 full-network updates
% \end{itemize}

% \subsection{Real-World Validation}
% Figure \ref{fig:wiki_results} extends these findings to Wikipedia-trained models, showing our curriculum approach improves:
% \begin{itemize}
%     \item MLM Accuracy: +18.4\% vs non-curriculum
%     \item Next Sentence Prediction: +12.7\%
% \end{itemize}

% The consistent gains across synthetic and real data confirm curriculum design--not just total bandwidth--drives distillation success.


% \paragraph{Discussion}
% PCFG

% \new{
% \begin{enumerate}
%     \item FLOPS -- compute efficiency and not time efficiency thing, but we gain. 
%     \item (potentially something about iteration) 
%     \item curriculum vs not.. we need curriculum, hidden rep has more info than just final layer and that is the reason our sechem works, but actually it is not enough to get info from final layer, intermediate layers help. 
%     -- hidden layer size our notion of bandwidth. 
% \end{enumerate}
% }

% wiki
% \new{
% -- look it works in practice, for real data. 
% }





% \subsection{Wikipedia}

% \subsection{n-gram PCFG}
% \label{subsec:PCFG}


% FIGURE BELOW: 

% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     \begin{minipage}[b]{0.8\linewidth}
%         \centering
%         \includegraphics[width=1\textwidth]{unpolished_figs/bert_pcfg_accuracy_In_progress.pdf}
%         \caption{BERT PCFG Accuracy}
%         \label{fig:mlp_student_accuracy}
%     \end{minipage}
%     % \begin{minipage}[b]{0.8\linewidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{unpolished_figs/parity_transformer_student_accuracy.pdf}
%     % \caption{MLP Student Accuracy}
%     % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     \hfill
%      \caption{(a) Layer-wise curriculum schedule showing progressive layer activation. (b) Validation accuracy on Wikipedia data, demonstrating curriculum benefits persist with real-world distributions.}
%     \label{fig:samples_vs_accuracy}.
% % \end{figure}

% \subsection{Curriculum Necessity}
% Figure \ref{fig:samples_vs_acc} reveals critical insights about knowledge distillation:

% \begin{itemize}
%     \item \textbf{Single-layer Failure}: Attempts using only the final transformer layer (dashed red) show catastrophic failure, achieving just 41.2\% accuracy vs 89.7\% for full curriculum
%     \item \textbf{Curriculum Advantage}: Our phased approach outperforms bandwidth-matched alternatives (68.4\% vs 89.7\%) despite equivalent total parameter updates
% \end{itemize}

%\section{Conclusion}
%In this work, we introduced a novel curriculum extraction scheme for knowledge distillation, in which the student network’s intermediate layers are trained to match a random projection of the hidden representations of the teacher network, before training using the full network. Theoretically, we show that this curriculum extraction strategy outperforms one-shot distillation when learning sparse parities using a two-layer MLP. Experimentally, our method consistently outperformed one-shot distillation on learning sparse parities, and on synthetic and real-world language modeling tasks.
%
%While our theory only applies to a stylized setting, one way to further justify our scheme could be to show similar performance gains for student learning under the hypothesis that high-level concepts that are of interest are represented linearly as directions in some representation space (i.e., the linear representation hypothesis). Also, our scheme uses random projections to extract a curriculum from the intermediate layers of the network, but there may be scope to improve performance by using a more sophisticated function to project down to the student hidden dimension, such as by making use of a trained autoencoder. We leave these as interesting directions for future work.

% \section*{Impact Statement}
% This work presents a memory-efficient alternative to progressive distillation by extracting a curriculum directly from the final teacher network. Smaller student models can help lower computational costs and energy consumption, thereby mitigating environmental impact. However, these benefits should be balanced against potential ethical concerns: if the teacher network contains biases or other undesirable characteristics, the distilled student may inherit or even amplify them. Therefore, responsible development and deployment of distilled models require careful auditing of teacher networks, transparent reporting of potential biases, and continual monitoring to ensure fairness and integrity.


% \subsection{BERT}
% \label{subsec:BERT}
% \paragraph{Masked Token Prediction:} Formally, let $v$ be a vocabulary (including the token \([mask]\)), and let $x$ be a sequence of length $h$. We randomly choose positions $M\subseteq [h]$ to mask, with each position included independently at probability $p$. We create a masked input $x \setminus M$ by replacing tokens in $M$ with \([mask]\), a random token, or leaving them unchanged with respective probabilities $80\%,\,10\%,\,10\%$.
% The model is then trained via a cross-entropy objective to predict the original tokens at those masked positions.

% \begin{figure}[t]
%     \centering
%     %--------------------
%     % First subfigure
%     %--------------------
%     % \begin{minipage}[b]{0.5\linewidth}
%         % \centering
%         \includegraphics[width=.9\linewidth]{}
%         \caption{BERT}
%         % \label{fig:mlp_student_accuracy}
%     % \end{minipage}
%     \hfill
%     \caption{%
%     \textbf{Curriculum Extraction vs Progressive Distillation.}
%     \emph{Left}: MLP on 100-dimensional 6-sparse parity, \new{with width-50k teachers and width-100 students.} }
%     \label{fig:mlp_sparse_parity}
% \end{figure}



% \section{Theoretical Guarantees for Sparse Parity}

% To demonstrate the effectiveness of our curriculum extraction scheme, we analyze it in the sparse parity function setting from \citep{panigrahi2024progressive}. We compare our two-stage training approach, which uses curriculum extraction based on a random projection of the hidden teacher dimension, to one-shot distillation, where the student is trained directly on teacher-generated samples. This section presents our main theorem (a formal version of \Cref{thm:main_informal}), outlines the proof, and briefly reviews key concepts and our setup.

% \subsection{Preliminaries}

% We study the performance of our curriculum extraction scheme in the context of learning the problem of sparse parities as defined in \Cref{prob:sparse_parities}. For our arguments, we will assume WLOG that the support of the unknown parity will be $S = [k]$. 

% % \begin{problem}[Learning Sparse Parities]
% % \label{prob:sparse_parities}
% %     Let \( S \subset [d] \) with \( |S| = k \) and \( k < d \). For \( \bx \in \{\pm 1\}^d \), define the label \( y_S \) to be $1$ if $\prod_{i \in S} x_i > 0$
% %     and $-1$ otherwise. 
% %     Given a tolerance \(\epsilon \in \R\) and $n$ samples \(\{(\bx_i, y(\bx_i)) \mid \bx_i \sim_{u.a.r} \{\pm 1\} \text{ for } i \in [0, n]\}\), 
% %     the objective is to learn a function \( f \) such that \(\| f - y_S \| \leq \epsilon\). 
% % \end{problem}


% The function $f$ that we will learn will be a two-layer neural networks: 
% $f(\bx) := \ba \cdot \sigma(\bW \cdot \bx + \bb) = \sum_{i=1}^m a_i \sigma(\bw_i \cdot \bx + b_i)$. 
% Here, $\bx \in \R^d, \bW \in \R^{d \times m}$ and $\bb, \ba \in \R^m$, and $\sigma(\cdot)$ is applied coordinate-wise.
% We will denote the student network by $f_s$ and the teacher network by $f_t$ with hidden dimensions $m_s$ and $m_t$ respectively.
% In general $m_s \ll m_t$. 

% In the next subsection, we describe our training setup. 

% \subsection{Training Setup}
% \label{subsec:training_setup}
% Prior to training, we will initialize the network using the following symmetric initialization from \citep{barak2022hidden}.

% \begin{definition}[Symmetric Initialization]
% \label{def:sym_initialization}
% Let $f(\bx) := \ba \cdot \sigma(\bW \cdot \bx + \mathbf{b})$ be a two-layer neural network with input dimension $d$ and hidden dimension $m$. 
% For each 
% $1 \leq i \leq m/2,$ $\bw_i \sim U(\{\pm 1\}^d),$ 
% $b_i \sim U\left(\left\{-1 + \frac{1}{k}, \cdots, 1 - \frac{1}{k}\right\}\right), 
% \quad a_i \sim U\left(\left\{\frac{\pm 1}{m}\right\}\right)$,
% $\bw_{i + m/2} = \bw_i, \quad b_{i + m/2} = b_i, \quad a_{i + m/2} = -a_i$
% \end{definition}


% \paragraph{Training Algorithms:}
% We train the teacher network $f_t$ by minimizing the hinge loss given by $\ell(\bx, y) := \max(0, 1-f_t(\bx)y)$ in two stages. 
% First, we freeze the top layer weights $(\ba)$ and train the network by with a regularized version of $\ell(\bx, y)$, given by $\ell(\bx, y) - \lambda \|\bW\|^2$ updating only $\bW, \bb$.
% In the second stage of training, we freeze the bottom layer weights $\bW$ and only update the weights in the top layer. 

% For the student network $f_s$, we define a \emph{distillation loss} instead.
% Let $f_T^{(1)} := \sigma(\bW \cdot \bx)$ denote the output of the first layer of the teacher and suppose $A \in \R^{m_t \times m_s}$ 
% is such that each $A_{ij} \sim U(\{\pm 1/m_t\})$. 
% In the first stage, the first layer ($f_s^{(1)}(\bx) := \sigma(\bW_s \cdot \bx + \bb)$) of the student is trained using the a similarly regularized version of the following hinge-like distillation loss: 
% \[
% \ell_{DL}(\bx, f_s^{(1)}, Af_t^{(1)}) = \max(0, 1 - f^{(1)}_s(\bx) \cdot Af^{(1)}_t(\bx)).
% \]
% The second layer of the student ($\ba_s$) is then trained using the standard hinge loss.



% \paragraph{Student Network:}
%     The student network is also a 2 layer neural network with the first layer having a smaller hidden dimension $m_s$.
%     $f_s(\bx) := \ba_s \cdot \sigma(\bW_s \cdot \bx)$, 
%     with $\ba_s \in \R^{m_s}$ and $\bW_s \in \R^{m_s \times d}$. 
    
% \paragraph{Student Training:}  
%     Let $f_T^{(1)} := \sigma(\bW \cdot \bx)$ denote the output of the first layer of the teacher and suppose $A \in \R^{m \times m_s}$ is such that each $A_{ij} \sim U(\{\pm 1/m\})$. 
%     The first layer ($f_s^{(1)}(\bx) := \sigma(\bW_s \cdot \bx)$) of the student is trained using the following hinge-like loss: 
%     \[
%     \ell_{DL}(x, f_s^{(1)}, Af_t^{(1)}) = \max(0, 1 - f^{(1)}_s(x) \cdot Af^{(1)}_t(x)).
%     \]
%     The second layer of the student ($\ba_s$) is then trained using the standard hinge loss.

% \paragraph{Learning Sparse Parities} The problem of learning a sparse parity is defined as follows:
% \begin{problem}[Learning Sparse Parities]
%     The problem of learning a sparse parity can be defined as follows: 
%     Let \( S \subset [d] \) with \( |S| = k \) and \( k < d \). For \( \bx \in \{\pm 1\}^d \), define the label \( y_S \) as:  
%     \[
%     y_S(\bx) = 
%     \begin{cases} 
%     1 & \text{if } \prod_{i \in S} x_i > 0, \\ 
%     -1 & \text{otherwise.}
%     \end{cases}
%     \]
%     Given samples $\epsilon \in \R$ and samples $\{(\bx_i, y(\bx_i)) \mid \bx_i \sim_{u.a.r} \{\pm 1\} \text{ for $i \in [0, n]$}\}$, the goal is to learn a function $f$ such that \new{$\| f - y_S\| \leq \epsilon$}.
%     \snote{What is the loss we use, exactly? The goal is likely just to minimize the hinge loss.}
% \end{problem}

% \paragraph{Function Class:} For theoretical illustration, we will try to learn sparse parities by two layer neural networks: $f(\bx) := \ba \cdot \sigma(\bW \cdot \bx) = \sum_{i=1}^m a_i \sigma(\bw_i \cdot \bx + b_i)$. 
% Here, $\bx \in \R^d, \bW \in \R^{d \times m}$ and $\ba \in \R^m$, 
% and $\sigma(\cdot)$ is applied coordinate-wise.

% We now describe our training setup. 

% \subsection{Training Setup}
% \label{subsec:training_setup}
% \paragraph{Initialization:} 
% We assume the data points are sampled at random from $U(\{\pm 1\}^d)$. Without loss of generality, let the target $k$-sparse parity function be $y = x_1 x_2 \cdots x_k$. Following (Barak et al., 2022), we use the following symmetric initialization: for each $1 \leq i \leq m/2$,
% $\bw_i \sim U(\{\pm 1\}^d), \quad b_i \sim U\left(\left\{-1 + \frac{1}{k}, \cdots, 1 - \frac{1}{k}\right\}\right), \quad a_i \sim U\left(\left\{\pm \frac{1}{m}\right\}\right),
%         \bw_{i + m/2} = \bw_i, \quad b_{i + m/2} = b_i, \quad a_{i + m/2} = -a_i$
%     % \begin{align}
%     %     \bw_i \sim U(\{\pm 1\}^d), \quad b_i \sim U\left(\left\{-1 + \frac{1}{k}, \cdots, 1 - \frac{1}{k}\right\}\right), \quad a_i \sim U\left(\left\{\pm \frac{1}{m}\right\}\right),\\
%     %     \bw_{i + m/2} = \bw_i, \quad b_{i + m/2} = b_i, \quad a_{i + m/2} = -a_i.
%     % \end{align}


% \paragraph{Teacher Network and training:}
% The teacher network is $f_t(\bx) := \ba \cdot \sigma(\bW \cdot \bx)$ with $\bx \in \R^d, \bW \in \R^{d \times m}$ and $\ba \in \R^m$.
% It is trained using hinge loss. 

    
% \paragraph{Student Network:}
%     The student network is also a 2 layer neural network with the first layer having a smaller hidden dimension $m_s$.
%     $f_s(\bx) := \ba_s \cdot \sigma(\bW_s \cdot \bx)$, 
%     with $\ba_s \in \R^{m_s}$ and $\bW_s \in \R^{m_s \times d}$. 
    
% \paragraph{Student Training:}  
%     Let $f_T^{(1)} := \sigma(\bW \cdot \bx)$ denote the output of the first layer of the teacher and suppose $A \in \R^{m \times m_s}$ is such that each $A_{ij} \sim U(\{\pm 1/m\})$. 
%     The first layer ($f_s^{(1)}(\bx) := \sigma(\bW_s \cdot \bx)$) of the student is trained using the following hinge-like loss: 
%     \[
%     \ell_{DL}(x, f_s^{(1)}, Af_t^{(1)}) = \max(0, 1 - f^{(1)}_s(x) \cdot Af^{(1)}_t(x)).
%     \]
%     The second layer of the student ($\ba_s$) is then trained using the standard hinge loss. 





% \Cref{thm:main} compares the sample complexity required by two strategies to train a student model to learn a \(k\)-sparse parity function over \(d\) variables --
% \textbf{random-projection curriculum extraction}, the one we propose in which we extract a curriculum and \textbf{one-shot distillation}, where the student is given samples from a trained teacher network.
% The theorem shows that curriculum extraction can be done in $O(2^{O(k)} \log(d)^2)$ samples while one-shot distillation reduces the sample complexity required to train the student network. 
% The core insight is that random projections of the first layer of the teacher model boost information about the support of the sparse parity, in the sense that each coordinate $h_i(\bx) := (Af_t^{(1)})_i(\bx)$ of the random projection of the first layer of the teacher network has \(\E_\bx[h_i(\bx) x_j]\) for \(j \in [k]\) much larger than \(\E_\bx[h_i(\bx) x_j]\) for \(j \notin [k]\), and this information can be easily transferred to the student network via the gradients (see \Cref{subsec:proof_overview}). 

% Note that if we directly try to used the outputs of the trained teacher network, this information cannot easily be found from the gradients of the loss, since the output of a sparse parity is uncorrelated with any other parity (including $x_i$). 





% \subsection{Proof Overview}
% \label{subsec:proof_overview}
% \Cref{item:necessary_one_shot_distill} in \Cref{thm:main} follows from the analogous result in \citep{panigrahi2024progressive} (Theorem B.1).
% The rest of this section will focus on the proof of \Cref{item:sufficient_our_distillation_scheme}.

% At a high level, the proof proceeds in two steps. We show that in \new{not too many}samples -- 
% (1) At the end of the first stage of student training, the learnt weight vectors have larger magnitudes in the coordinates in the support of $S$.
% (2) At the end of the second stage of training, the final network is a good predictor of the underlying parity function. 

% To show point (1), the core insight is that random projections of the first layer of the teacher model contain information about the support of the sparse parity, in the sense that each coordinate $h_i(\bx) := (Af_t^{(1)})_i(\bx)$ is such that $\E_\bx[h_i(\bx) x_j]$ for $j \in [k]$ is much larger than $\E_\bx[h_i(\bx) x_j]$ for $j \notin [k]$. Once this is established, 
% \snote{here}
% \Cref{prop:fourier_gap_implies_recovery} from \citep{barak2022hidden}  (stated below) implies that this information can be extracted by the first layer of the student network directly from the gradient updates. 

% \new{give some intuition for why there should be a gap.. }

% \begin{proposition}[(Proposition 9 from \citep{barak2022hidden}) Fourier gap implies feature recovery]
% \label{prop:fourier_gap_implies_recovery}
% For an activation function \(\phi : \mathbb{R} \to \mathbb{R}\), let \(f(x; w) = \phi(w \cdot x)\) be the corresponding 1-neuron predictor. 
% Let \(D_S\) be an \((n, k)\)-sparse parity distribution. Let \(g(w)\) be an estimate for the neuron's population gradient of the \new{correlation loss:}
% \[
% \| g(w) -  \mathbb{E}_{(x, y) \sim D_S} \left[ \nabla_w \ell(y, f(w;x))\right] \|_\infty \leq \gamma/2 ,
% \]
% Then, for every \(w\) such that \(\phi(w \cdot x)\) has a Fourier gap at \(S\), the \(k\) 
% indices at which \(g(w)\) has the largest absolute values are exactly the indices in \(S\).
% \end{proposition}



% \begin{proof}
%     The bounds on $c_S$ for $S \subset [n]$ follow from \Cref{lem:bounds_on_coeffs,lem:even_deg_coeffs}.
%     \new{SK: need to combine the lemmas and add the norm bound stuff for this to work.}
%     The proof of the second part follows analogously to Corollary B.6 from \citep{panigrahi2024progressive}.
% \end{proof}

	
	\section{Preliminaries}
	Notation:
	\begin{enumerate}
		\item We will use $\langle f, g \rangle$ to mean $\E_{x \sim \{\pm 1\}^d} [f(x)g(x)]$, and $\langle f, g \rangle_D := \E_{x \sim D} [f(x)g(x)]$. 
		\item The correlation loss is given by $\ell_c(f , y) := \E_{(x, y)}[f(x)y]$, where $(x, y)$ are draw from a distribution that will be clear from context.  
	\end{enumerate}
	


\subsection{Calculations}
	
\paragraph{Setup:}	For some even number $r$, we consider a ReLU MLP of size $r$:
	\[ f(x;\theta) := \sum_{i=1}^r u_i \sigma(w_i^T x + b_i).\]
	Here, $\theta := \{ w_1, \dots, w_r, b, u\}$ where $w_1, \dots, w_r \in \R^n$, $b \in \R^r$ and $u \in \R^r$. 
	WLOG assume $S = [k]$ and $y = \Pi_{i=1}^k x_i$. 
	\begin{enumerate}
	\item For all $1 \leq i \leq r/2$ randomly initialize, 
	$w_i^{0} \sim \text{Unif}(\{\pm 1\}^n), u_i^{0} \sim \text{Unif}(\{\pm 1\}), b_i^{0} \sim \text{Unif}(\{-1+1/k, \dots, 1-1/k\})$. 
	\item For all $r/2 < i \leq r$, initialize 
	$w_i^{(0)} = w_{i-r/2}^{(0)}, b_i^{0} = b_{i-r/2}^{(0)}, u_i^{(0)} = -u_{i-r/2}^{(0)}$. 
	\end{enumerate}

\paragraph{Gradient Calculations:}
We will re-use some of the gradient calculations from \cite{}. For ease of reference, we bundle them together in the following lemma
\begin{lemma}
	\begin{enumerate}
		\item The population gradient is given by, 
		\begin{equation}\label{eq:pop_grad_w}
			g_{i,j} = \E [\nabla_{w_{i, j}} l(f(x;\theta_0), y)] = u_i \E[y\mathbf{1}\{w_i \cdot x + b_i \geq 0\} x_j], 
		\end{equation}
	and 
		\begin{equation}
		\E [\nabla_{b_i} l(f(x;\theta_0), y)] = u_i \E[y\mathbf{1}\{w_i \cdot x + b_i \geq 0\}].
	\end{equation}
	\item Let $y(x) = \Pi_{i \in S} (x_i + \eps_i) + g(x)$ where $\E_{x}[g^2(x)] \leq n^{-c}$ and 
	$\eps_i \sim_{u.a.r} \{ -\eps, \eps\}$. 
	\end{enumerate}
\end{lemma}
\begin{proof}
	Substituting for $y$ in \Cref{eq:pop_grad_w}, and an application of Cauchy-Schwartz implies,
	\begin{align*}
		g_{i,j} 
		&= u_i \E[ \Pi_{i \in S} (x_i + \eps_i) \mathbf{1}\{w_i \cdot x + b_i \geq 0\} x_j] + u_i \E[ g(x) \mathbf{1}\{w_i \cdot x + b_i \geq 0\} x_j]\\
		&= u_i \E[ \Pi_{i \in S} (x_i + \eps_i) \mathbf{1}\{w_i \cdot x + b_i \geq 0\} x_j] \pm n^{-c/2}\\
		&= u_i \E\left [ \left (\sum_{T \subseteq S} \left( \prod_{i \in T} \epsilon_i \prod_{i \in S \setminus T} x_i \right) \right) \mathbf{1}\{w_i \cdot x + b_i \geq 0\} x_j \right] \pm n^{-c/2}\\
		&= u_i \sum_{T \subseteq S} \E\left [ \left (\sum_{T \subseteq S} \left( \prod_{i \in T} \epsilon_i \prod_{i \in S \setminus T} x_i \right) \right) \mathbf{1}\{w_i \cdot x + b_i \geq 0\} x_j \right] \pm n^{-c/2}\\
	\end{align*}
	Focusing on $u_i \E[ \Pi_{i \in S} (x_i + \eps_i) \mathbf{1}\{w_i \cdot x + b_i \geq 0\} x_j$, 
\end{proof}
	

\section{Theoretical Guarantees}
In \cite{}, the authors demonstrate that the network \( f_T^{(1)}(x) \), after the first phase of training, satisfies a Fourier gap. This gap is a sufficient condition for SGD to rapidly converge to the underlying minimizer. 

We consider the network after training, denoted \( f_T^{(2)}(\cdot) \), and replace its top-layer weights with weights drawn from the initialization distribution specified in \Cref{eqn:initialization}. We refer to the resulting network as \( f_T^r(\cdot) \).

The outline of our proof is as follows. We show that, with constant probability, 
$\mathbb{E}_{x} \big[f_T^r(x) x_i\big]$
is noticeably larger for \( i \in S \) compared to \( i \notin S \). This guarantees that the gap property from \cite{} holds, ensuring faster convergence. Let $\zeta_i = \mathbb{E}_{x, y}\big[\text{Maj}(x) \chi_S(x)\big],
$
for any \( S \subseteq \{0, 1\}^d \) with \( |S| = i \). It is known that \( \zeta_i = 0 \) when \( i \) is even, and \( \zeta_i = \Theta\left(\frac{i^{-1/3}}{\binom{d}{i}}\right) \) when \( i \) is odd \cite{}.

\begin{lemma}[Lemma B.2 (Single step gradient descent, from \cite{} and adapted from Claims 1, 2 in Barak et al. (2022))] 
Fix \( \tau_g, \delta > 0 \). Set \( T_1 = 1 \). Suppose the batch size \( B_1 \geq \Omega(\tau_g^{-2} \log(md/\delta)) \). For learning rate \( \eta_1 = \frac{m}{k |\zeta_{k-1}|} \) and \( \lambda_1 = 1 \), the following conditions hold true for all neurons \( i \in [m] \) at the end of the first stage of training with probability at least \( 1 - \delta \).

\begin{enumerate}
    \item \( \left| w^{(1)}_{ij} - \frac{\operatorname{sign}(a^{(0)}_i \zeta_{k-1}) \operatorname{sign}(\chi_{[k] \setminus \{j\}}(w^{(0)}_i))}{2k} \right| \leq \frac{\tau_g}{|\zeta_{k-1}|}, \) for all \( j \in [k] \).
    
    \item \( \left| w^{(1)}_{ij} - \frac{\zeta_{k+1}}{|\zeta_{k-1}|} \frac{\operatorname{sign}(a^{(0)}_i) \operatorname{sign}(\chi_{[k] \cup \{j\}}(w^{(0)}_i))}{2k} \right| \leq \frac{\tau_g}{|k \zeta_{k-1}|}, \) for all \( j > k \).
\end{enumerate}
\end{lemma}

Substituting for the value of $\zeta_{i}$, this essentially means
$|w_{ij}^{(1)}| = \frac 1 {2k} \pm \frac {\tau_g \cdot \binom{d}{k-1} } {(k-1)^{-1/3}}$ for $j \in [k]$,
and $|w_{ij}^{(1)}| = \frac {(k+1)^2} {2k~d^2} (1-\frac 2 {k+1})^{1/3} (1+\frac 2 {k-1})^{k-1} \pm \frac {\tau_g \cdot \binom{d}{k-1} } {k (k-1)^{-1/3}}$ otherwise. 

\begin{fact}[Fourier Expansion of $\relu$]
    $\relu(\sum_{i=1}^m w_i x_i + b) = $
\end{fact}

\begin{lemma}[Expansion of $f_T^r(\cdot)$]

\end{lemma}

\begin{lemma}[Gap Property]
\( \mathbb{E}_{x,y} \left[ f^{r}_T(x) x_i \right] 
\geq \frac{1}{8k} + O\left( \tau_{gd} |\zeta_{k-1}|^{-1} \right) + O(m^{-1/2}) \) for all \( i \in S \).
\end{lemma}

\begin{theorem}[Main Theorem]

\end{theorem}
\begin{proof}


The population gradient of the weight vector in neuron \(i\) at coordinate \(j\) is given by:

\[
\mathbb{E}_{x, y} \nabla_{\tilde{w}_{ij}^{(0)}} \ell_{\text{DL}}(x, y; f_S^{(0)}, f_T^r) 
= -\mathbb{E}_{x, y} \nabla_{\tilde{w}_{ij}^{(0)}} f_S^{(0)}(x) f_T^{r}(x).
\]

Expanding this, we get:
\[
-\mathbb{E}_{x, y} \nabla_{\tilde{w}_{ij}^{(0)}} f_S^{(0)}(x) f_T^{r}(x) 
= -a_i \mathbb{E}_{x, y} \Big[I\big(\langle \tilde{w}_i^{(0)}, x \rangle + \tilde{b}_i \geq 0\big) f_T^{r}(x) x_j\Big],
\]
where \(I(\cdot)\) is the indicator function. \new{Using the relationship between \(I\big(\langle \tilde{w}_i^{(0)}, x \rangle + \tilde{b}_i \geq 0\big)\) and \(\text{Maj}(\tilde{w}_i^{(0)}, x)\)}, we rewrite the expression as:
\[
-\frac{a_i}{2} \mathbb{E}_{x, y} \big[f^r_T(x) x_j\big] 
- \frac{a_i}{2} \mathbb{E}_{x, y} \big[\text{Maj}(\tilde{w}_i^{(0)} \cdot x) f^r_T(x) x_j\big].
\]

The relationship between \(I\big(\langle \tilde{w}_i^{(0)}, x \rangle + \tilde{b}_i \geq 0\big)\) and \(\text{Maj}(\tilde{w}_i^{(0)}, x)\) holds because \(|\tilde{b}_i| < 1\) at initialization.

\end{proof}




\begin{lemma}[Lemma B.5 from \cite{} (Correlation with in-support variables)]
Under the event that the conditions in Lemma B.2 are satisfied by each neuron, which occurs with probability at least \(1 - \delta\) with respect to the randomness of initialization and sampling, the output of the model after the first phase satisfies the following conditions:

\begin{enumerate}
    \item \( \mathbb{E}_{x,y} \left[ f^{(1)}_T(x) x_i \right] \geq \frac{1}{8k} + O\left( \tau_{gd} |\zeta_{k-1}|^{-1} \right) + O(m^{-1/2}) \) for all \( i \in S \).
    
    \item \( \mathbb{E}_{x,y} \left[ f^{(1)}_T(x) x_i \right] \leq O\left( (kd)^{-1} \right) \) for all \( i \notin S \).
    
    \item \( \mathbb{E}_{x,y} \left[ f^{(1)}_T(x) \chi_S(x) \right] \leq O\left( \tau_{gd} |\zeta_{k-1}|^{-1} \right) \) for all \( S \) with even \( |S| \).
    
    \item \( \left\| f^{(1)}_T \right\|_2^2 = \mathbb{E}_{x,y} \left[ \left( f^{(1)}_T(x) \right)^2 \right] \leq O\left( \frac{d}{k} \right) \).
\end{enumerate}

\comment{
\textbf{Corollary B.6}. Under the event that the conditions in Lemma B.2 are satisfied by each neuron, which occurs with probability at least \( 1 - \delta \) with respect to the randomness of initialization and sampling, the output of the model after the first phase can be given as:
\[
f^{(1)}_T(x) = \sum_{j=1}^{k} c_j x_j + \sum_{j=k+1}^{d} c_j x_j + \sum_{\substack{S \subseteq [d] \\ |S| \% 2 = 1, |S| \geq 3}} c_S \chi_S(x) + \sum_{\substack{S \subseteq [d] \\ |S| \% 2 = 0}} c_S \chi_S(x),
\]
where
\[
|c_j| \geq \Omega\left(\frac{1}{k}\right), \quad \text{for all } 1 \leq j \leq k,
\]
\[
|c_j| \leq O\left(\frac{1}{kd}\right), \quad \text{for all } j > k,
\]
\[
|c_S| \leq O\left(\tau_{gd} |\zeta_{k-1}|^{-1}\right), \quad \text{for all } S \subseteq [d] \text{ with } |S| \% 2 = 0,
\]
\[
|c_S| \leq O\left(\frac{d}{k}\right), \quad \text{for all } S \subseteq [d] \text{ with } |S| \% 2 = 1.
\]

As such, the following correlations hold true for all \( i \):
\[
\mathbb{E}_{x,y} \left[ f^{(1)}_T(x) \cdot \operatorname{Maj}(x) x_i \right] = \frac{1}{2} c_i + O\left(\tau_{gd}^{5/3} |\zeta_{k-1}|^{-1}\right).
\]

If batch size \( B_1 \) is set such that \( B_1 \geq \Omega\left(k^2 d^{10/3} \zeta_{k-1}^{-2}\right) \) and \( \tau_g \leq O\left(k^{-1} d^{-5/3} |\zeta_{k-1}|\right) \), then the following holds for all \( i \):
\[
\mathbb{E}_{x,y} \left[ f^{(1)}_T(x) \cdot \operatorname{Maj}(x) x_i \right] \geq \Omega\left(\frac{1}{k}\right), \quad \text{if } i \in [k],
\]
\[
\mathbb{E}_{x,y} \left[ f^{(1)}_T(x) \cdot \operatorname{Maj}(x) x_i \right] \leq o\left(\frac{1}{k}\right), \quad \text{if } i \notin [k].
\]


\begin{theorem}[Sample complexity benefits with progressive distillation]
Suppose the teacher model has been trained with 2-stage training in Algorithm 1, which satisfies the conditions in Corollary B.6 at the end of the first stage and achieves loss \(O(d^{-c})\) for some constant \(c \geq 1\) at the end of the second stage. Suppose we train a student model \(f_S\) of size \(\tilde{m} = \Theta(2^{\tilde{k} k})\) using the following two strategies:
\begin{enumerate}
    \item \textbf{Progressive distillation:} Train for the first \(T_1 = 1\) steps with respect to the teacher’s logits at \(T_1\) checkpoint. Then, train with the final teacher checkpoint in the second stage.
    \item \textbf{Distillation:} Train with the final teacher checkpoint throughout training.
\end{enumerate}
Then,
\begin{enumerate}
    \item Under progressive distillation, the total sample complexity to reach a loss of \(\epsilon\) with probability \(1 - \delta\) is
    \[
    \Theta\left( k^2 \log\left(\frac{dm}{\tilde{\delta}}\right) + 2k d^2 k^4 \epsilon^{-2} \log\left(\frac{k}{\delta}\right) \right).
    \]
    \item The necessary sample complexity under distillation is at least
    \[
    \Omega\left( d^{\min(2c, k-1)} \right).
    \]
\end{enumerate}
\end{theorem}




	First observe that  
		Our proof proceeds in two steps. 
	First, we show that after updating the weights using the gradients, 
	the resulting weights are close to $1/2k$. 
	Then, we show that there exist values for $u_1, \dots, u_r$ such that
	the resulting function is close to the unknown sparse parity. 
	Since searching for $u_1, \dots, u_r$ is a convex program, 
	our result will follow. We first state our update:
	
	\paragraph{Update:}
	Assume we randomly initialize an MLP using the unbiased initialization defined previously.
	
	\begin{equation} \label{eq:w_update}
		w^{(1)}_i = (1 - \lambda_0)w^{(0)}_i - \eta_0 \hat g_i
	\end{equation}
	
	\begin{equation} \label{eq:b_update}
		b^{(1)}_i = b^{(0)}_i - \eta_0 \hat \gamma_i
	\end{equation}
	
	where
	
	\begin{equation} \label{eq:gradient_g}
		\hat g_i = \frac{1}{B} \sum_{l=1}^{B} \nabla_{w_i} \ell(f(x_{0,l}; \theta_0), y_{0,l}),
	\end{equation}
	
	\begin{equation} \label{eq:gradient_gamma}
		\hat \gamma_i = \frac{1}{B} \sum_{l=1}^{B} \nabla_{b_i} \ell(f(x_{0,l}; \theta_0), y_{0, l})
	\end{equation}

	Also, define 
		
	\begin{equation} \label{eq:pop_gradient_g}
		 g_i =\E_{(x, y)}[\nabla_{w_i} \ell(f(x; \theta_0), y)]
	\end{equation}
	
	\begin{equation} \label{eq:pop_gradient_gamma}
		 \gamma_i = \E_{(x, y)}[ \nabla_{b_i} \ell(f(x; \theta_0), y)]
	\end{equation}
	
	
	
	We will need the following calculations. 
	First, we show that the gradient can help us identify the
	coordinates in $S$. 
	Recall that for the first stage, we have 
	
	
	\begin{lemma}
		Assume $k$ is even and $n \geq 2(k+1)^2$. 
		Let $y(x) = \Pi_{j \in S} c_j + \sum_{j \in S} x_j c_j + \sum_{j,k \in S, j \neq k} x_j x_k c_{j} c_k + $
		Then the following hold, 
		\begin{enumerate}
			\item If $j \in S$ then: 
			\item If $j \notin S$ then: 
			\item $\gamma_i = 0$. 
		\end{enumerate}
	\end{lemma}
	\begin{proof}
		
	\end{proof}
	
	
	
	\begin{claim}[Updated weights are close to uniform]
	Consider the case where $\lambda_0 = 1$ and $\eta_0 = ??$ in \Cref{eq:w_update}.
	Then, for all $i$ and $j \in S$ we have $w^{(1)}_{i,j} = \frac{1}{2k} \pm ??$. 
	\end{claim}
	\begin{proof}
		
	\end{proof}
	
	
	\begin{fact}
		Suppose a function $f$ satisfies $\langle f(x), \chi_S(x) \rangle \geq 1-2\eps$. 
	\end{fact}
	
	\begin{fact}
		Let $\eta_1, \dots, \eta_d$ be drawn iid from $\{ \pm 1/2 \}$, 
		then $\langle \chi_S(x+\eta), x_i \rangle \geq 1/4$. 
	\end{fact}
	
	
	\begin{lemma}[Sample Complexity for Gradient Information]
		
	\end{lemma}
	
	
	\begin{lemma}[Existence of a Good $u$]
		
	\end{lemma}
	
}

